Conditional independence testing under misspecified inductive biases

Conditional independence (CI) testing is a fundamental and challenging task in modern statistics and machine learning. Many modern methods for CI testing rely on powerful supervised learning methods to learn regression functions or Bayes predictors as an intermediate step; we refer to this class of tests as regression-based tests. Although these methods are guaranteed to control Type-I error when the supervised learning methods accurately estimate the regression functions or Bayes predictors of interest, their behavior is less understood when they fail due to misspecified inductive biases; in other words, when the employed models are not flexible enough or when the training algorithm does not induce the desired predictors. Then, we study the performance of regression-based CI tests under misspecified inductive biases. Namely, we propose new approximations or upper bounds for the testing errors of three regression-based tests that depend on misspecification errors. Moreover, we introduce the Rao-Blackwellized Predictor Test (RBPT), a regression-based CI test robust against misspecified inductive biases. Finally, we conduct experiments with artificial and real data, showcasing the usefulness of our theory and methods.

==> YK-macros.tex <==
\usepackage{dsfont}

\def\Avar{{\sf Avar}}
\def\abs#1{\left|#1\right|}
\def\aff{{\sf aff}}
\def\argmin{{\arg\min}}
\def\argmax{{\arg\max}}
\def\avar{{\sf avar}}

%\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
%\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}

\def\bA{\mathbf{A}}
\def\bB{\mathbf{B}}
\def\bC{\mathbf{C}}
\def\bD{\mathbf{D}}
\def\bE{\mathbf{E}}
\def\bF{\mathbf{F}}
\def\bff{\mathbf{f}}
\def\bG{\mathbf{G}}
\def\bH{\mathbf{H}}
\def\bI{\mathbf{I}}
\def\bJ{\mathbf{J}}
\def\bK{\mathbf{K}}
\def\bL{\mathbf{L}}
\def\bM{\mathbf{M}}
\def\bN{\mathbf{N}}
\def\bO{\mathbf{O}}
\def\bP{\mathbf{P}}
\def\bQ{\mathbf{Q}}
\def\bR{\mathbf{R}}
\def\bS{\mathbf{S}}
\def\bT{\mathbf{T}}
\def\bU{\mathbf{U}}
\def\bV{\mathbf{V}}
\def\bW{\mathbf{W}}
\def\bX{\mathbf{X}}
\def\bY{\mathbf{Y}}
\def\bZ{\mathbf{Z}}

\def\bGamma{{\boldsymbol\Gamma}}
\def\bDelta{{\boldsymbol\Delta}}
\def\bTheta{{\boldsymbol\Theta}}
\def\bLambda{{\boldsymbol\Lambda}}
\def\bXi{{\boldsymbol\Xi}}
\def\bPi{{\boldsymbol\Pi}}
\def\bSigma{{\boldsymbol\Sigma}}
\def\bUps{{\boldsymbol\Upsilon}}
\def\bPhi{{\boldsymbol\Phi}}
\def\bPsi{{\boldsymbol\Psi}}
\def\bOmega{{\boldsymbol\Omega}}

\def\ba{\mathbf{a}}
\def\bb{\mathbf{b}}
\def\bc{\mathbf{c}}
\def\bbd{\mathbf{d}}
\def\bd{{\sf bd}}
\def\be{\mathbf{e}}
\def\bbf{\mathbf{f}}
\def\bg{\mathbf{g}}
\def\bh{\mathbf{h}}
\def\bi{\mathbf{i}}
\def\bj{\mathbf{j}}
\def\bk{\mathbf{k}}
\def\bl{\mathbf{l}}
% \def\bm{\mathbf{m}}
\def\bn{\mathbf{n}}
\def\bo{\mathbf{o}}
\def\bp{\mathbf{p}}
\def\bq{\mathbf{q}}
\def\br{\mathbf{r}}
\def\bs{\mathbf{s}}
\def\bt{\mathbf{t}}
\def\bu{\mathbf{u}}
\def\bv{\mathbf{v}}
\def\bw{\mathbf{w}}
\def\bx{\mathbf{x}}
\def\by{\mathbf{y}}
\def\bz{\mathbf{z}}

\def\balpha{{\boldsymbol\alpha}}
\def\bbeta{{\boldsymbol\beta}}
\def\bgamma{{\boldsymbol\gamma}}
\def\bdelta{{\boldsymbol\delta}}
\def\beps{{\boldsymbol\epsilon}}
\def\bveps{{\boldsymbol\varepsilon}}
\def\bzeta{{\boldsymbol\zeta}}
\def\bfeta{{\boldsymbol\eta}}
\def\btheta{{\boldsymbol\theta}}
\def\bvtheta{{\boldsymbol\vartheta}}
\def\biota{{\boldsymbol\iota}}
\def\bkappa{{\boldsymbol\kappa}}
\def\blambda{{\boldsymbol\lambda}}
\def\bmu{{\boldsymbol\mu}}
\def\bnu{{\boldsymbol\nu}}
\def\bxi{{\boldsymbol\xi}}
\def\bpi{{\boldsymbol\pi}}
\def\brho{{\boldsymbol\rho}}
\def\bvrho{{\boldsymbol\varrho}}
\def\bsigma{{\boldsymbol\sigma}}
\def\btau{{\boldsymbol\tau}}
\def\bups{{\boldsymbol\upsilon}}
\def\bphi{{\boldsymbol\phi}}
\def\bvphi{{\boldsymbol\varphi}}
\def\bpsi{{\boldsymbol\psi}}
\def\bomega{{\boldsymbol\omega}}

\def\bbA{\mathbb{A}}
\def\bbB{\mathbb{B}}
\def\bbC{\mathbb{C}}
\def\bbD{\mathbb{D}}
\def\bbE{\mathbb{E}}
\def\bbF{\mathbb{F}}
\def\bbG{\mathbb{G}}
\def\bbH{\mathbb{H}}
\def\bbI{\mathbb{I}}
\def\bbJ{\mathbb{J}}
\def\bbK{\mathbb{K}}
\def\bbL{\mathbb{L}}
\def\bbM{\mathbb{M}}
\def\bbN{\mathbb{N}}
\def\bbO{\mathbb{O}}
\def\bbP{\mathbb{P}}
\def\bbQ{\mathbb{Q}}
\def\bbR{\mathbb{R}}
\def\bbS{\mathbb{S}}
\def\bbT{\mathbb{T}}
\def\bbU{\mathbb{U}}
\def\bbV{\mathbb{V}}
\def\bbW{\mathbb{W}}
\def\bbX{\mathbb{X}}
\def\bbY{\mathbb{Y}}
\def\bbZ{\mathbb{Z}}

\def\Ber{{\sf Ber}}
\def\bin{{\sf bin}}

\def\cA{\mathcal{A}}
\def\cB{\mathcal{B}}
\def\cC{\mathcal{C}}
\def\cD{\mathcal{D}}
\def\cE{\mathcal{E}}
\def\cF{\mathcal{F}}
\def\cG{\mathcal{G}}
\def\cH{\mathcal{H}}
\def\cI{\mathcal{I}}
\def\cJ{\mathcal{J}}
\def\cK{\mathcal{K}}
\def\cL{\mathcal{L}}
\def\cM{\mathcal{M}}
\def\cN{\mathcal{N}}
\def\cO{\mathcal{O}}
\def\cP{\mathcal{P}}
\def\cQ{\mathcal{Q}}
\def\cR{\mathcal{R}}
\def\cS{\mathcal{S}}
\def\cT{\mathcal{T}}
\def\cU{\mathcal{U}}
\def\cV{\mathcal{V}}
\def\cW{\mathcal{W}}
\def\cX{\mathcal{X}}
\def\cY{\mathcal{Y}}
\def\cZ{\mathcal{Z}}

\def\cat{{\sf cat}}
\def\Cov{{\sf Cov}}
\def\cov{{\sf cov}}
\def\card{{\bf card}}
\def\cf{{\it cf.}}
\def\cl{{\sf cl}}
\def\complex{{\bbC}}
\def\cone{{\sf cone}}
\def\conv{{\sf conv}}
\def\deq{\overset{d}{=}}
\def\det{{\sf det}}
\def\diag{{\sf diag}}
\def\diam{{\sf diam}}
\def\dist{{\sf dist}}
\def\dom{{\sf dom}}
\def\doop{{\sf do}}
\def\dto{\overset{\sf d}{\to}}
\def\Ex{{\bbE}}
\def\Exp{{\sf Exp}}
\def\exp{{\sf exp}}
\def\eg{{\it e.g.}}
\def\epi{{\sf epi}}
\def\eps{{\epsilon}}
\def\etc{{\it etc.}}
\def\ie{{\it i.e.}}
\def\iid{{\sf iid}}
\def\ind{{\sf ind}}
\def\intr{{\sf int}}
\def\integers{{\bbZ}}

\def\halpha{\widehat{\balpha}}
\def\hbeta{\widehat{\bbeta}}
\def\hdelta{\widehat{\bdelta}}
\def\hGamma{\widehat{\bGamma}}
\def\hgamma{\widehat{\bgamma}}
\def\hmu{\widehat{\bmu}}
\def\hSigma{\widehat{\bSigma}}
\def\hsigma{\widehat{\bsigma}}
\def\hTheta{\widehat{\bTheta}}
\def\htheta{\widehat{\btheta}}
\def\hw{\widehat{\bw}}

\def\KL{{\sf KL}}
\def\ker{{\sf ker}}
\def\lspan{{\sf span}}
\def\maximize{{\sf maximize}}
\def\med{{\sf med}}
\def\minimize{{\sf minimize}}
\def\norm#1{\left\|#1\right\|}
\def\ones{\mathds{1}}
\def\Poi{{\sf Poi}}
\def\Pr{{\bbP}}
\def\peq{\overset{\sf p}{=}}
\def\plim{{\sf plim}}
\def\proj{{\sf proj}}
\def\prox{{\sf prox}}
\def\pto{\overset{\sf p}{\to}}
\def\ran{{\sf ran}}
\def\rank{{\sf rank}}
\def\reals{{\bbR}}
\def\relint{{\sf relint}}
\def\sign{{\sf sign}}
\def\supp{{\sf supp}}
\def\symm{{\bbS}}

\def\st{\textrm{subject to}}
\def\tr{{\sf tr}}
\def\tube{{\sf tube}}
\def\TV{{\sf TV}}
\def\unif{{\sf unif}}
\def\Var{{\sf Var}}
\def\var{{\sf var}}
\def\vct{{\sf vec}}
\def\veps{\varepsilon}
\def\vol{{\sf vol}}
\def\zeros{\mathbf{0}}


==> YK-thm-macros.tex <==

\newtheorem{theorem}{Theorem}[section]
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{model}[theorem]{Model}
% \newenvironment{proof}{\noindent {\sc Proof:}}{$\Box$ \medskip} 
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{remark}[theorem]{Remark}


==> append.tex <==
\section{Extra content}

\subsection{Examples on when STFR fails}\label{append:examples}

Examples \ref{ex:counter_example1} and  \ref{ex:counter_example2} show simple situations in which Type-I error control is compromised or the conditional independence test has no power due to model misspecification. As we see in the next examples, Type-I error control is directly related to $\cG_2$ misspecification, while Type-II error minimization directly relates to $\cG_1$ misspecification. 


\begin{example}[No Type-I error control]\label{ex:counter_example1}
Suppose $Y=Z+Z^2+\varepsilon_y$ and $X=Z^2+\varepsilon_x$, where $\varepsilon_y, \varepsilon_x \sim N(0,1)$ are independent noise variables and $Z$ has finite variance. Consequently, $X \indep Y \mid Z$. Let $\cG_1$ and $\cG_2$ be the classes of linear regressors with no intercept, i.e., $$\cG_1=\{g_1(x,z)=\beta_x x+\beta_z z: \beta_x, \beta_z\in\reals\} \text{ and } \cG_2=\{g_2(z)=\beta_z z:  \beta_z\in\reals\}.$$
If $\ell$ denotes the mean squared error,  we have that $\Ex_P [\ell (g^*_{2,P}(Z),Y)] - \Ex_P [\ell (g^*_{1,P}(X,Z),Y)]  > 0$ because the model class $\cG_2$ is misspecified, that is, it does not contain the Bayes predictor given by the conditional expectation $\Ex [Y\mid Z]$.
\end{example}

\begin{example}[Powerless test]\label{ex:counter_example2}
Suppose $Y=Z+\sin(X)+\varepsilon_y$, where $Z,X,\varepsilon_y \overset{iid}{\sim} N(0,1)$. Consequently, $X \not\indep Y \mid Z$. Define $\cG_1$ and $\cG_2$ as in Example \ref{ex:counter_example1}. If $\ell$ denotes the mean squared error,  we have that\footnote{Because $\Ex_P[XY]=\Ex_P[X\Ex_P[Y|X]]=\Ex_P[X\cdot 0]=0$.} $\Ex _P[\ell (g^*_{2,P}(Z),Y)] - \Ex_P [\ell (g^*_{1,P}(X,Z),Y)]  = 0$ even though the different Bayes' predictors have a difference in performance. This happens because 
the model $g^*_{1,P}$ is not close enough to the Bayes predictor $\Ex_P [Y\mid X,Z]$.
\end{example}



\subsection{REgression with Subsequent Independence Test (RESIT)}\label{append:resit}


As revisited by \citet{zhang2017feature}, the idea behind RESIT is to first residualize $Y$ and $X$ given $Z$ and then test dependence between the residuals. It is similar to GCM, but requires the error terms and $Z$ to be independent. When that assumption is reasonable, one advantage of RESIT over GCM is that it has power against a broader set of alternatives. In this section, we use a permutation test \citep[Example 15.2.3]{lehmann2005testing} to assess the independence of residuals. We analyse RESIT's Type-I error control.


If $(X,Y,Z)\sim P$ and $(X,Y)$ can be modeled as an additive noise model (ANM), that is, we can write 
\begin{align}\label{eq:anm}
    X=f_{1,P}^*(Z)+\epsilon ~~\text{ and }~~ Y=f_{2,P}^*(Z)+\eta,
\end{align}
where $f_{1,P}^*(Z)=\Ex_P[X\mid Z]$, $f_{2,P}^*(Z)=\Ex_P[Y\mid Z]$, and the error terms $(\epsilon,\eta)$ are independent of $Z$, it is possible to show that $X \indep Y \mid Z \Leftrightarrow \epsilon \indep \eta.$
To facilitate our analysis\footnote{In practice, data splitting is not necessary. However, this procedure helps when theoretically analyzing the method.}, we consider first fitting two models $\hat{g}^{(m)}_{1}$ and $\hat{g}^{(m)}_{2}$ that approximate $f^*_{1,P}$ and $f^*_{2,P}$ using the training set $\cD^{(m)}_{tr}$ and then test the independence of the residuals\footnote{We omit the residuals superscript to ease notation.} $\hat{\epsilon}_i=X_i-\hat{g}^{(m)}_{1}(Z_i)$ and $\hat{\eta}_i=Y_i-\hat{g}^{(m)}_{2}(Z_i)$ using the test set $\cD^{(n)}_{te}$. Define (i) $(\boldsymbol{\hat{\epsilon}},\boldsymbol{\hat{\eta}})\triangleq\{(\hat{\epsilon}_i,\hat{\eta}_i)\}_{i=1}^n$ (test set residuals vertically stacked in matrix form) and (ii) $(\boldsymbol{\hat{\epsilon}},\boldsymbol{\hat{\eta}})^{(b)}$ as one of the $B$ permutations, \ie, consider that we fix $\boldsymbol{\hat{\epsilon}}$ and permute $\boldsymbol{\hat{\eta}}$ row-wise. Let $\Psi$ be a test statistic and $\Psi((\boldsymbol{\hat{\epsilon}},\boldsymbol{\hat{\eta}}))$ and $\Psi((\boldsymbol{\hat{\epsilon}},\boldsymbol{\hat{\eta}})^{(b)})$ its evaluation on the original residuals and the $b$-the permuted set. If the permutation $p$-value is given by 
\begin{align}\label{eq:anm_pval}
    p(\cD^{(n)}_{te}, \cD^{(m)}_{tr})=\frac{1+\sum_{b=1}^B\ones[\Psi((\boldsymbol{\hat{\epsilon}},\boldsymbol{\hat{\eta}})^{(b)})\geq\Psi((\boldsymbol{\hat{\epsilon}},\boldsymbol{\hat{\eta}}))]}{1+B}
\end{align}
a test $\varphi^{\textup{RESIT}}_\alpha$ aiming level $\alpha \in (0,1)$ is given by Equation \ref{eq:test_STFR}. 

Similarly to STFR and GCM, we consider $g_{1,P}^*$ and $g_{2,P}^*$ to be the limiting models for $\hat{g}^{(m)}_{1}$ and $\hat{g}^{(m)}_{2}$. Different from GCM, both models $g_{1,P}^*$ and $g_{2,P}^*$ are multi-output since $X$ and $Y$ are not necessarily univariate. 

Now, we introduce some assumptions before we present our result for RESIT. Assumption \ref{assump:assump1_resit} gives a rate of convergence for the models $\hat{g}_{j}^{(m)}$ in the mean squared error sense.
\begin{assumption}\label{assump:assump1_resit}
    There are models $g_{1,P}^*$, $g_{2,P}^*$, and a constant $\gamma>0$ such that
    \begin{align*}
       \Ex_P\left[\norm{\hat{g}_{j}^{(m)}(Z)- g^*_{j,P}(Z)}_2^2 \Big |~ \cD_{tr}^{(m)}\right]=\cO_{\cP_0}(m^{-\gamma}), ~~j=1,2
    \end{align*}
\end{assumption}

Assumption \ref{assump:assump2_resit} puts more structure on the distributions of the error terms $(\epsilon,\eta)$ and is a mild assumption. 
\begin{assumption}\label{assump:assump2_resit}
    Assume that for all $P \in \cP_0$, the distribution of $(\epsilon,\eta)$, $P_{\epsilon,\eta}$, is absolutely continuous with respect to the Lebesgue measure in $\reals^{d_X }\times \reals^{d_Y}$ with $L$-Lipschitz density $p_{\epsilon,\eta}$ for a certain $L>0$. That is, for any $e_1,e_2 \in \reals^{d_X}$ and $h_1,h_2 \in \reals^{d_Y}$, we have
    \begin{align*}
        &|p_{\epsilon,\eta}(e_1,h_1)-p_{\epsilon,\eta}(e_2,h_2)|\leq L\norm{(e_1,h_1)-(e_2,h_2)}_2
    \end{align*}
    We assume that $L$ does not depend on $P$.
\end{assumption}

Assumption \ref{assump:assump3_resit} states that some of the variables we work with are uniformly almost surely bounded over all $P\in\cP_0$. This assumption is realistic in most practical cases.
\begin{assumption}\label{assump:assump3_resit}
    There is bounded Borel set $A \in \cB(\reals^{d_X\times d_Y})$ such that
    \[
    \inf_{P \in \cP_0}\Pr_P\left((X,Y) \in A \right)=1
    \]
    and 
    \[
    \inf_{P \in \cP_0}\inf_{g_1,g_2}\Pr_P\left((g_1(Z),g_2(Z)) \in A \right)=1
    \]
\end{assumption}

Here, $\inf_{g_1,g_2}$ is taken over the model classes we consider (if the model classes vary with $m$, consider the union of model classes). In the following, we present the result for RESIT. For that result, let: (i) $\epsilon^* \triangleq \epsilon -\delta_{1,P}(Z_i)$ and $\eta^*\triangleq \eta -\delta_{2,P}(Z_i)$, where the misspecification gaps are given as in Definition \ref{def:gaps2}; (ii) $d_\text{TV}$ represent the total variation (TV) distance between two probability distributions \citep{tsybakov2004introduction2}; and (iii) the superscript  $n$, \eg, in $P^n_{\epsilon^*,\eta^*}$, represent a product measure.

\begin{theorem}\label{thm:thm1_resit}
    Under Assumptions \ref{assump:assump1_resit}, \ref{assump:assump2_resit}, and \ref{assump:assump3_resit}, if $H_0:X\indep Y\mid Z$ holds and $n$ is a function of $m$ such that $n\to \infty$ and $n=o(m^\frac{\gamma}{2})$ as $m\to \infty$,  then
    \begin{align*}
    \Ex_P[\varphi^{\textup{RESIT}}_\alpha(\cD^{(n)}_{te}, \cD^{(m)}_{tr})]\leq \alpha + \min\{d_\text{TV}(P^n_{\epsilon^*,\eta^*},P^n_{\epsilon,\eta^*}), d_\text{TV}(P^n_{\epsilon^*,\eta^*},P^n_{\epsilon^*,\eta})\} +o(1)
    \end{align*}
    where $o(1)$ denotes uniform convergence over all $P \in \cP_0$ as $m\to \infty$.
\end{theorem}

From Theorem \ref{thm:thm1_resit}, we can see that if at least one of the  misspecification gaps $\delta_{1,P}$ or $\delta_{2,P}$ is null, then $\Ex_P[\varphi^{\textup{RESIT}}_\alpha(\cD^{(n)}_{te}, \cD^{(m)}_{tr})]\leq \alpha$ under $H_0:X\indep Y\mid Z$. This can be seen as a \textit{double-robustness} property of the RESIT. If none of the misspecification gaps are null, we do not have any guarantees on RESIT's Type-I error control. It can be shown that the proposed upper bound converges to $1$. 


\subsection{RBPT extra derivation}\label{append:rbpt}

Let $\mu_X$ be a dominating measure of $Q^*_{X\mid Z}$ and $P_{X\mid Z}$ that does not depend on $Z$. Let $q^*_{X\mid Z},p_{X\mid Z}$ be $Q^*_{X|Z},P_{X\mid Z}$ densities with respect to $\mu_X$.
\begin{align*}
 \Omega_{P,1}^{\textup{RBPT}}&=\Ex_P\Bigg[\ell\left(\int  g_{P}^{*}(x,Z) dQ^*_{X|Z}(x),Y\right)- \ell\left(\int  g_{P}^{*}(x,Z) dP_{X\mid Z}(x),Y\right) \Bigg]\\
 &\leq L \cdot\Ex_P\norm{\int  g_{P}^{*}(x,Z) dQ^*_{X|Z}(x) -\int  g_{P}^{*}(x,Z) dP_{X\mid Z}(x)}_2\\
 &\leq L\cdot\Ex_P\norm{\int  g_{P}^{*}(x,Z) dQ^*_{X|Z}(x) -\int  g_{P}^{*}(x,Z) dP_{X\mid Z}(x)}_1\\
 &= L\cdot\Ex_P\norm{\int  g_{P}^{*}(x,Z) (q^*_{X|Z}(x|Z) -p_{X\mid Z}(x|Z))d\mu_{X}(x)}_1\\
 &\leq  L\cdot\Ex_P\int  \norm{g_{P}^{*}(x,Z)}_1 |q^*_{X|Z}(x|Z) -p_{X\mid Z}(x|Z)|d\mu_{X}(x)\\
 &\leq  ML\cdot\Ex_P\int   |q^*_{X|Z}(x|Z) -p_{X\mid Z}(x|Z)|d\mu_{X}(x)\\
 &=  2ML\cdot\Ex_P[d_\text{TV}(Q^*_{X|Z},P_{X\mid Z})]
\end{align*}
If
\[
 \Ex_P[d_\text{TV}(Q^*_{X|Z},P_{X\mid Z})]\leq \Omega_{P,2}^{\textup{RBPT}}/(2ML)
\]
then
\[
 \Omega^{\textup{RBPT}}_{P}\leq0
\]



\subsection{How to obtain a result for RBPT2?}\label{append:rbpt2}

We informally give some ideas on extending Theorem \ref{thm:thm1_rbpt}. Theorem \ref{thm:thm1_rbpt} states that

\begin{align*}
\Ex_P[\varphi^{\textup{RBPT}}_\alpha(\cD^{(n)}_{te},\cD_{tr}^{(m)})]=1-\Phi\left(\tau_{\alpha}-\sqrt{\frac{n}{\sigma_P^2}}\Omega_P^{\textup{RBPT}}\right) +o(1)
\end{align*}
where $\Omega_P^{\textup{RBPT}}=\Omega_{P,1}^{\textup{RBPT}}-\Omega_{P,2}^{\textup{RBPT}}$
with
\begin{align*}
   \Omega_{P,1}^{\textup{RBPT}}\triangleq \Ex_{P}&\Bigg[\ell\left(\int  g_{P}^{*}(x,Z) dQ^*_{X|Z}(x),Y\right)\Bigg]- \Ex_{P}\Bigg[\ell\left(\int  g_{P}^{*}(x,Z) dP_{X\mid Z}(x),Y\right) \Bigg]
\end{align*}
and
\begin{align*}
   \Omega_{P,2}^{\textup{RBPT}}\triangleq \Ex_{P}&\big[\ell(g_{P}^*(X,Z),Y)\big]- \Ex_{P}\Bigg[\ell\left(\int g_{P}^*(x,Z) dP_{X\mid Z}(x),Y\right) \Bigg] 
\end{align*}

If we wanted to adapt that result for RBPT2, we would have to redefine $\Omega_{P,1}^{\textup{RBPT}}$. The analogue of $\Omega_{P,1}^{\textup{RBPT}}$ for RBPT2 would be 
\begin{align*}
   \Omega_{P,1}^{\textup{RBPT2}}\triangleq \Ex_{P}&\Bigg[\ell\left(\Tilde{\Ex}_P\left[g_{P}^{*}(X,Z)\mid Z\right] ,Y\right)\Bigg]- \Ex_{P}\Bigg[\ell\left(\Ex_P\left[g_{P}^{*}(X,Z)\mid Z\right] ,Y\right) \Bigg]
\end{align*}
where $\Tilde{\Ex}_P\left[g_{P}^{*}(X,Z)\mid Z=z\right]$ denotes the limiting regression model to predict $g_{P}^{*}(X,Z)$ given $Z$. If we assume the existence of a big unlabeled dataset, deriving a result might be easier as we can avoid the asymptotic details on the convergence of the second regression model by assuming that the limiting Rao-Blackwellization model, for a fixed initial predictor, is known. The only challenge is proving the convergence of $\Tilde{\Ex}_P\left[\hat{g}(X,Z)\mid Z\right]$ to $\Tilde{\Ex}_P\left[g_{P}^{*}(X,Z)\mid Z\right]$. With the proper assumptions and sufficient structure, the result can be achieved.



\subsection{Model misspecification in modern statistics and machine learning: an experiment}\label{append:missp}

This study demonstrates that the control of Type-I error by the Generalized Covariance Model (GCM) test \citep{shah2020hardness} is contingent on the training algorithm and not only on the model classes. We work in the context of a high-dimensional (overparameterized) regression problem with a training set of 250 observations and 500 covariates. The data are generated as follows:
\[
Z\sim N(0,I_{500}), ~~~ X\mid Z \sim N(\beta_X^\top Z, 1), ~~~ Y\mid X,Z \sim N(\beta_Y^\top Z, 1)
\]

where the first five entries of $\beta_X$ are set to 20, and the remaining entries are zero, while the last five entries of $\beta_Y$ are set to 20, and the remaining entries are zero. This results in $X$ and $Y$ being conditionally independent given $Z$ and depending on $Z$ only through a small number of entries. Additionally, $\Ex[X\mid Z]=\beta_X^\top Z$ and $\Ex[Y\mid Z]=\beta_Y^\top Z$, indicating that the linear model class is correctly specified. To perform the GCM test, we use LASSO ($\norm{\cdot}_1$ penalization term added to empirical squared error) and the minimum-norm least-squares solution \citep{arora2019theory} to fit linear models that predict $X$ and $Y$ given $Z$. In this problem, the LASSO fitting approach provides the correct inductive bias since $\beta_X$ and $\beta_Y$ are sparse. 

To conduct the experiment, we set $\alpha=10\%$, sample a training set, and fit the models. Then, we sample 500 test sets to estimate the Type-I error rate. Repeating this process for 100 different training sets, we obtain a distribution of the Type-I error rates for each fitting method. Figure \ref{fig:linear_model_experiment} illustrates that, despite using the same model class for both fitting methods, the training algorithm induces model misspecification in the minimum-norm case, implying an invalid test most of the time.

\begin{figure}[h]
    \centering
    \includegraphics[width=.4\textwidth]{Neurips_2023/figs/linear_model_exp.png}
    \caption{Type-I error by the GCM test is contingent on the training algorithm used and not solely on the model classes. The figure shows the distribution of Type-I error rates for LASSO and the minimum-norm least-squares solution, obtained by sampling 500 test sets for each fitting method and repeating the process for 100 different training sets. The results demonstrate that the minimum-norm solution model is misspecified due to the training algorithm, which often renders the GCM test invalid.}
    \label{fig:linear_model_experiment}
\end{figure}

\newpage
\section{Technical proofs}\label{append:proofs}

\subsection{STFR }

\begin{lemma}\label{lemma:lemma1_stfr}
Assume we are under the conditions of Theorem \ref{thm:thm1_stfr}. Then:
\[
(\hat{\sigma}^{(n,m)})^2 - \Var_P[T^{(m)}_1\mid  \cD_{tr}^{(m)}]=o_\cP(1) \text{ as } m\to \infty
\]
\begin{proof}
First, see that for an arbitrary $\varepsilon>0$, there must be\footnote{Because of the definition of $\sup$.} a sequence of probability measures in $\cP$, $(P^{(m)})_{m\in\mathbb{N}}$, such that
\begin{align*}
   &\sup_{P\in \cP}\Pr_P\left[\left|(\hat{\sigma}^{(n,m)})^2-  \Var_P[T^{(m)}_1\mid  \cD_{tr}^{(m)}]\right|>\varepsilon\right]\leq \Pr_{P^{(m)}}\left[\left|(\hat{\sigma}^{(n,m)})^2-  \Var_{P^{(m)}}[T^{(m)}_1\mid  \cD_{tr}^{(m)}]\right|>\varepsilon\right] + \frac{1}{m}
\end{align*}
Pick one of such sequences. Then, to prove that $(\hat{\sigma}^{(n,m)})^2 - \Var_P[T^{(m)}_1\mid  \cD_{tr}^{(m)}]=o_\cP(1) \text{ as } m\to \infty$, it suffices to show that
\[
\Pr_{P^{(m)}}\left[\left|(\hat{\sigma}^{(n,m)})^2-  \Var_{P^{(m)}}[T^{(m)}_1\mid  \cD_{tr}^{(m)}]\right|>\varepsilon\right] \to 0 \text{ as }m\to \infty
\]

Now, expanding $(\hat{\sigma}^{(n,m)})^2$ we get
\begin{align*}
    (\hat{\sigma}^{(n,m)})^2&= \frac{1}{n}\sum_{i=1}^n (T^{(m)}_i)^2-\left(\frac{1}{n}\sum_{i=1}^n T^{(m)}_i\right)^2\\
    &=\frac{1}{n}\sum_{i=1}^n \left[(T^{(m)}_i)^2- \Ex_{P^{(m)}}[(T^{(m)}_1)^2\mid  \cD_{tr}^{(m)}] \right]+ \Ex_{P^{(m)}}[(T^{(m)}_1)^2\mid  \cD_{tr}^{(m)}]-\left(\frac{1}{n}\sum_{i=1}^n T^{(m)}_i\right)^2\\
    &=\frac{1}{n}\sum_{i=1}^n \left[(T^{(m)}_i)^2- \Ex_{P^{(m)}}[(T^{(m)}_1)^2\mid  \cD_{tr}^{(m)}] \right]-\left(\frac{1}{n}\sum_{i=1}^n T^{(m)}_i- \Ex_{P^{(m)}}[T^{(m)}_1\mid  \cD_{tr}^{(m)}]\right)^2\\
    &~~~~ -2\left(\frac{1}{n}\sum_{i=1}^n T^{(m)}_i\Ex_{P^{(m)}}[T^{(m)}_1\mid  \cD_{tr}^{(m)}]- (\Ex_{P^{(m)}}[T^{(m)}_1\mid  \cD_{tr}^{(m)}])^2\right)+ \Var_{P^{(m)}}[T^{(m)}_1\mid  \cD_{tr}^{(m)}]\\
    &=\frac{1}{n}\sum_{i=1}^n \left[(T^{(m)}_i)^2- \Ex_{P^{(m)}}[(T^{(m)}_1)^2\mid  \cD_{tr}^{(m)}] \right]-\left(\frac{1}{n}\sum_{i=1}^n T^{(m)}_i- \Ex_{P^{(m)}}[T^{(m)}_1\mid  \cD_{tr}^{(m)}]\right)^2\\
    &~~~~ -2\Ex_{P^{(m)}}[T^{(m)}_1\mid  \cD_{tr}^{(m)}]\left(\frac{1}{n}\sum_{i=1}^n T^{(m)}_i- \Ex_{P^{(m)}}[T^{(m)}_1\mid  \cD_{tr}^{(m)}]\right)+ \Var_{P^{(m)}}[T^{(m)}_1\mid  \cD_{tr}^{(m)}]
\end{align*}

Then,
\begin{align*}
    &(\hat{\sigma}^{(n,m)})^2 - \Var_{P^{(m)}}[T^{(m)}_1\mid  \cD_{tr}^{(m)}]=\\
    &=\frac{1}{n}\sum_{i=1}^n \left[(T^{(m)}_i)^2- \Ex_{P^{(m)}}[(T^{(m)}_1)^2\mid  \cD_{tr}^{(m)}] \right]-\left(\frac{1}{n}\sum_{i=1}^n T^{(m)}_i- \Ex_{P^{(m)}}[T^{(m)}_1\mid  \cD_{tr}^{(m)}]\right)^2\\
    &~~~~ -2\Ex_{P^{(m)}}[T^{(m)}_1\mid  \cD_{tr}^{(m)}]\left(\frac{1}{n}\sum_{i=1}^n T^{(m)}_i- \Ex_{P^{(m)}}[T^{(m)}_1\mid  \cD_{tr}^{(m)}]\right)
\end{align*}

Using a law of large numbers for
triangular arrays \citep[Corollary 9.5.6]{cappe2009inference} (we comment on needed conditions to use this result below) and the continuous mapping theorem, we have that
\begin{itemize}
    \item $\frac{1}{n}\sum_{i=1}^n \left[(T^{(m)}_i)^2- \Ex_{P^{(m)}}[(T^{(m)}_1)^2\mid  \cD_{tr}^{(m)}] \right]=o_p(1)$
    \item $\left(\frac{1}{n}\sum_{i=1}^n T^{(m)}_i- \Ex_{P^{(m)}}[T^{(m)}_1\mid  \cD_{tr}^{(m)}]\right)^2=o_p(1)$
    \item $\underbrace{2\Ex_{P^{(m)}}[T^{(m)}_1\mid  \cD_{tr}^{(m)}]}_{\cO_p(1)\text{ (Assumption \ref{assump:assump2_stfr})}}\left(\frac{1}{n}\sum_{i=1}^n T^{(m)}_i- \Ex_{P^{(m)}}[T^{(m)}_1\mid  \cD_{tr}^{(m)}]\right)=o_{p}(1)$
\end{itemize}

and then
\begin{align*}
   &\sup_{P\in \cP}\Pr_P\left[\left|(\hat{\sigma}^{(n,m)})^2-  \Var_P[T^{(m)}_1\mid  \cD_{tr}^{(m)}]\right|>\varepsilon\right]\leq \Pr_{P^{(m)}}\left[\left|(\hat{\sigma}^{(n,m)})^2-  \Var_{P^{(m)}}[T^{(m)}_1\mid  \cD_{tr}^{(m)}]\right|>\varepsilon\right] + \frac{1}{m} \to 0
\end{align*}
 $\text{ as }m\to \infty$, i.e.,
\[
(\hat{\sigma}^{(n,m)})^2 - \Var_P[T^{(m)}_1\mid  \cD_{tr}^{(m)}]=o_\cP(1) \text{ as } m\to \infty
\]

\textit{Conditions to use the law of large numbers.} Let $(P^{(m)})_{m\in\mathbb{N}}$ be an arbitrary sequence of probability measures in $\cP$. Define our triangular arrays as $\left\{V^{(m)}_{i,1}\right\}_{1 \leq i \leq n}$ and $\left\{V^{(m)}_{i,2}\right\}_{1 \leq i \leq n}$, where
$V^{(m)}_{i,1}\triangleq T^{(m)}_i- \Ex_{P^{(m)}}[T^{(m)}_1\mid  \cD_{tr}^{(m)}]$ and $V^{(m)}_{i,2}\triangleq (T^{(m)}_i)^2- \Ex_{P^{(m)}}[(T^{(m)}_1)^2\mid  \cD_{tr}^{(m)}]$. Now, we comment on the conditions for the law of large numbers \citep[Corollary 9.5.6]{cappe2009inference}:
\begin{enumerate}
    \item This condition naturally applies by definition and because of Assumption \ref{assump:assump2_stfr}.

    \item  From Assumption \ref{assump:assump2_stfr} and \citet[Example 6.5.2]{resnick2019probability}, 
    \begin{align*}
       \Ex_{P^{(m)}}\left[\left|V^{(m)}_{i,1}\right| \mid  \cD_{tr}^{(m)}\right]\leq \Ex_{P^{(m)}}\left[\left|T^{(m)}_i\right| \mid  \cD_{tr}^{(m)}\right]+ \left|\Ex_{P^{(m)}}[T^{(m)}_1\mid  \cD_{tr}^{(m)}]\right| \leq 2\Ex_{P^{(m)}}\left[\left|T^{(m)}_i\right| \mid  \cD_{tr}^{(m)}\right]=\cO_p(1)
    \end{align*}
    and 
    \begin{align*}
       \Ex_{P^{(m)}}\left[\left|V^{(m)}_{i,2}\right| \mid  \cD_{tr}^{(m)}\right]\leq 2\Ex_{P^{(m)}}\left[(T^{(m)}_i)^2 \mid  \cD_{tr}^{(m)}\right]=\cO_p(1)
    \end{align*}

    \item Fix any $\epsilon>0$ and let $k$ be defined as in Assumption \ref{assump:assump2_stfr}. See that
    \begin{align*}
        \Ex_{P^{(m)}}\left[\left| V^{(m)}_{i,1} \right| \ones[|V^{(m)}_{i,1}|\geq \epsilon n] \mid  \cD_{tr}^{(m)}\right] 
        &= \Ex_{P^{(m)}}\left[\left| V^{(m)}_{i,1} \right| \ones[(|V^{(m)}_{i,1}|/(\epsilon n))^{k}\geq 1] \mid  \cD_{tr}^{(m)}\right]\\
        &\leq \frac{1}{(n\epsilon)^{k}} \Ex_{P^{(m)}}\left[|V^{(m)}_{i,1}|^{1+k}\mid  \cD_{tr}^{(m)}\right]\\
        &= \frac{1}{(n\epsilon)^{k}} \Ex_{P^{(m)}}\left[|T^{(m)}_i- \Ex_{P^{(m)}}[T^{(m)}_1\mid  \cD_{tr}^{(m)}]|^{1+k}\mid  \cD_{tr}^{(m)}\right]\\
        &\leq \frac{1}{(n\epsilon)^{k}} \left\{\Ex_{P^{(m)}}\left[|T^{(m)}_i|^{1+k}\mid  \cD_{tr}^{(m)}\right]^{\frac{1}{1+k}} + \Ex_{P^{(m)}}\left[|T^{(m)}_i|\mid  \cD_{tr}^{(m)}\right] \right\}^{1+k}\\
        &= \frac{1}{(n\epsilon)^{k}} \cO_p(1)\\
        &= o_p(1)
    \end{align*}
    where the third inequality is obtained via Minkowski Inequality \citep{resnick2019probability} and the fifth step is an application of Assumption \ref{assump:assump2_stfr} and \citet[Example 6.5.2]{resnick2019probability}. Analogously, define $k'=k/2$ and see that
    \begin{align*}
        \Ex_{P^{(m)}}\left[\left| V^{(m)}_{i,2} \right| \ones[|V^{(m)}_{i,2}|\geq \epsilon n] \mid  \cD_{tr}^{(m)}\right]
        &= \Ex_{P^{(m)}}\left[\left| V^{(m)}_{i,2} \right| \ones[(|V^{(m)}_{i,2}|/(\epsilon n))^{k'}\geq 1] \mid  \cD_{tr}^{(m)}\right]\\
        &\leq \frac{1}{(n\epsilon)^{k'}} \Ex_{P^{(m)}}\left[|V^{(m)}_{i,2}|^{1+k'}\mid  \cD_{tr}^{(m)}\right]\\
        &= \frac{1}{(n\epsilon)^{k'}} \Ex_{P^{(m)}}\left[|(T^{(m)}_i)^2- \Ex_{P^{(m)}}[(T^{(m)}_1)^2\mid  \cD_{tr}^{(m)}]|^{1+k'}\mid  \cD_{tr}^{(m)}\right]\\
        &\leq \frac{1}{(n\epsilon)^{k'}} \left\{\Ex_{P^{(m)}}\left[(T^{(m)}_i)^{2(1+k')}\mid  \cD_{tr}^{(m)}\right]^{\frac{1}{1+k'}} + \Ex_{P^{(m)}}\left[(T^{(m)}_i)^2\mid  \cD_{tr}^{(m)}\right] \right\}^{1+k'}\\
        &= \frac{1}{(n\epsilon)^{k'}} \left\{\Ex_{P^{(m)}}\left[(T^{(m)}_i)^{2+k}\mid  \cD_{tr}^{(m)}\right]^{\frac{1}{1+k'}} + \Ex_{P^{(m)}}\left[(T^{(m)}_i)^2\mid  \cD_{tr}^{(m)}\right] \right\}^{1+k'}\\
        &= \frac{1}{(n\epsilon)^{k'}} \cO_p(1)\\
        &= o_p(1)
    \end{align*} 
\end{enumerate}

\end{proof}
\end{lemma}


\textbf{Theorem \ref{thm:thm1_stfr}.} Suppose that Assumptions \ref{assump:assump1_stfr}, \ref{assump:assump2_stfr}, and \ref{assump:assump3_stfr} hold. If $n$ is a function of $m$ such that $n\to \infty$ and $n=o(m^{2\gamma})$ as $m\to \infty$,  then
\begin{align*}
\Ex_P[\varphi^{\textup{STFR}}_\alpha(\cD^{(n)}_{te},\cD_{tr}^{(m)})]=1-\Phi\left(\tau_{\alpha}-\sqrt{\frac{n}{\sigma_P^2}}\Omega_P^{\textup{STFR}}\right) +o(1)
\end{align*}
where $o(1)$ denotes uniform convergence over all $P \in \cP$ as $m\to \infty$ and
\[
\Omega_P^{\textup{STFR}}\triangleq \Ex_P[\ell(g^*_{2,P}(Z),Y)]-\Ex_P[\ell(g^*_{1,P}(X,Z),Y)]
\]
\begin{proof}
First, note that there must be\footnote{Because of the definition of $\sup$.} a sequence of probability measures in $\cP$, $(P^{(m)})_{m\in\mathbb{N}}$, such that
\begin{align*}
   &\sup_{P\in \cP}\left|\Ex_P[\varphi^{\textup{STFR}}_\alpha(\cD^{(n)}_{te},\cD_{tr}^{(m)})]-1+\Phi\left(\tau_{\alpha}-\sqrt{\frac{n}{\sigma_P^2}}\Omega_P^{\textup{STFR}}\right)\right|\leq \left|\Ex_{P^{(m)}}[\varphi^{\textup{STFR}}_\alpha(\cD^{(n)}_{te},\cD_{tr}^{(m)})]-1+\Phi\left(\tau_{\alpha}-\sqrt{\frac{n}{\sigma_{P^{(m)}}^2}}\Omega_{P^{(m)}}^{\textup{STFR}}\right)\right| + \frac{1}{m}
\end{align*}

Then, it suffices to show that the RHS vanishes when we consider such a sequence $(P^{(m)})_{m\in\mathbb{N}}$.

Now, let us first decompose the test statistic $\Lambda^{(n,m)}$ in the following way:
\begin{align*}
&\Lambda^{(n,m)}\triangleq\\
&\triangleq\frac{\sqrt{n}\bar{T}^{(n,m)}}{\hat{\sigma}^{(n,m)}}\\
&=\frac{\sqrt{n}\Big(\bar{T}^{(n,m)}-\Ex_{P^{(m)}}[T^{(m)}_1 \mid \cD_{tr}^{(m)}]\Big)}{\hat{\sigma}^{(n,m)}}+\frac{\sqrt{n}\Ex_{P^{(m)}}[T^{(m)}_1 \mid \cD_{tr}^{(m)}]}{\hat{\sigma}^{(n,m)}}\\
    &=\frac{\sqrt{n}\Big(\bar{T}^{(n,m)}-\Ex_{P^{(m)}}[T^{(m)}_1 \mid \cD_{tr}^{(m)}]\Big)}{\hat{\sigma}^{(n,m)}}+\\
    &~~+ \frac{\sqrt{n}\Big(\Ex_{P^{(m)}}[\ell(\hat{g}_{2}^{(m)}(Z_1),Y_1)-\ell(g_{2,P^{(m)}}^*(Z_1),Y_1)\mid \cD_{tr}^{(m)}]-\big(\Ex_{P^{(m)}}[\ell(\hat{g}_{1}^{(m)}(X_1,Z_1),Y_1)-\ell(g_{1,P^{(m)}}^*(X_1,Z_1),Y_1)\mid \cD_{tr}^{(m)}]\big)\Big)}{\hat{\sigma}^{(n,m)}}\\
    &~~+ \frac{\sqrt{n}\Big(\Ex_{P^{(m)}}[\ell(g_{2,P^{(m)}}^*(Z_1),Y_1)]-\Ex_{P^{(m)}}[\ell(g_{1,P^{(m)}}^*(X_1,Z_1),Y_1)]\Big)}{\hat{\sigma}^{(n,m)}}\\
    &=\frac{\sqrt{n}W^{(m)}_{1, P^{(m)}}}{\hat{\sigma}^{(n,m)}}+\frac{\sqrt{n}W^{(m)}_{2, P^{(m)}}}{\hat{\sigma}^{(n,m)}}+\frac{\sqrt{n} \Omega_{P^{(m)}}^{\textup{STFR}}}{\hat{\sigma}^{(n,m)}}
\end{align*}

Given that $n$ is a function of $m$, we omit it when writing the $W^{(m)}_{j, P^{(m)}}$'s. Define $\sigma_{P^{(m)}}^{(m)}\triangleq \sqrt{\Var_{P^{(m)}}[T^{(m)}_1\mid  \cD_{tr}^{(m)}]}$ and see that
\begin{align}
    \Ex_{P^{(m)}}[\varphi^{\textup{STFR}}_\alpha(\cD^{(n)}_{te},\cD_{tr}^{(m)}) ]&=\Pr_{P^{(m)}}[p(\cD^{(n)}_{te},\cD_{tr}^{(m)})\leq \alpha] \nonumber\\
    &=\Pr_{P^{(m)}}\left[1-\Phi\left(\Lambda^{(n,m)}\right)\leq \alpha \right] \nonumber\\
    &=\Pr_{P^{(m)}}\left[\Lambda^{(n,m)} \geq \tau_\alpha \right] \nonumber\\
    &=\Pr_{P^{(m)}}\left[\frac{\sqrt{n}W^{(m)}_{1, P^{(m)}}}{\hat{\sigma}^{(n,m)}}+\frac{\sqrt{n}W^{(m)}_{2, P^{(m)}}}{\hat{\sigma}^{(n,m)}}+\frac{\sqrt{n}\Omega_{P^{(m)}}^{\textup{STFR}}}{\hat{\sigma}^{(n,m)}} \geq \tau_\alpha\right] \nonumber\\
    &=\Pr_{P^{(m)}}\left[\frac{\sqrt{n}W^{(m)}_{1, P^{(m)}}}{\sigma_{P^{(m)}}}+\frac{\sqrt{n}W^{(m)}_{2, P^{(m)}}}{\sigma_{P^{(m)}}}+\frac{\sqrt{n}\Omega_{P^{(m)}}^{\textup{STFR}}}{\sigma_{P^{(m)}}} + \tau_\alpha- \tau_\alpha \frac{\hat{\sigma}^{(n,m)}}{\sigma_{P^{(m)}}}\geq \tau_\alpha \right] \nonumber\\
    &=\Pr_{P^{(m)}}\left[\frac{\sqrt{n}W^{(m)}_{1, P^{(m)}}}{\sigma_{P^{(m)}}^{(m)}}\frac{\sigma_{P^{(m)}}^{(m)}}{\sigma_{P^{(m)}}}+\frac{\sqrt{n}W^{(m)}_{2, P^{(m)}}}{\sigma_{P^{(m)}}} + \tau_\alpha- \tau_\alpha \frac{\hat{\sigma}^{(n,m)}}{\sigma_{P^{(m)}}^{(m)}}\frac{\sigma_{P^{(m)}}^{(m)}}{\sigma_{P^{(m)}}}\geq \tau_\alpha -\frac{\sqrt{n}\Omega_{P^{(m)}}^{\textup{STFR}}}{\sigma_{P^{(m)}}}\right] \nonumber\\
    %&=\Pr_{P^{(m)}}\left[\frac{\sqrt{n}W^{(m)}_{1, P^{(m)}}}{\sigma_{P^{(m)}}^{(m)}} \geq \tau_\alpha - \sqrt{\frac{n}{\sigma_{P^{(m)}}^2}}\Omega_{P^{(m)}}^{\textup{STFR}} \right]+o(1) \label{step:step1_stfr}\\
    &=1-\Phi\left(\tau_\alpha -\sqrt{\frac{n}{\sigma_{P^{(m)}}^2}}\Omega_{P^{(m)}}^{\textup{STFR}}\right)+o(1)\label{step:step1_stfr}
\end{align}

Implying that
\begin{align*}
   &\sup_{P\in \cP}\left|\Ex_P[\varphi^{\textup{STFR}}_\alpha(\cD^{(n)}_{te},\cD_{tr}^{(m)})]-1+\Phi\left(\tau_{\alpha}-\sqrt{\frac{n}{\sigma_P^2}}\Omega_P^{\textup{STFR}}\right)\right|= o(1) \text{ as }m\to \infty
\end{align*}

\textit{Justifying step \ref{step:step1_stfr}.} First, from a central limit theorem for triangular arrays \citep[Corollary 9.5.11]{cappe2009inference}, we have that
\[
\sqrt{n}\left(\frac{W^{(m)}_{1, P^{(m)}}}{\sigma_{P^{(m)}}^{(m)}}\right)= \sqrt{n}\left(\frac{\bar{T}^{(n,m)}-\Ex_{P^{(m)}}[T^{(m)}_1 \mid \cD_{tr}^{(m)}]}{\sigma_{P^{(m)}}^{(m)}}\right) = \frac{1}{\sqrt{n}}\sum_{i=1}^n\left(\frac{T_i^{(m)}-\Ex_{P^{(m)}}[T^{(m)}_1 \mid \cD_{tr}^{(m)}]}{\sigma_{P^{(m)}}^{(m)}}\right)\Rightarrow N(0,1)
\]
we comment on the conditions to use this theorem below.

Second, we have that
\begin{align*}
   &\frac{\sqrt{n}W^{(m)}_{1, P^{(m)}}}{\sigma_{P^{(m)}}^{(m)}}- \left(\frac{\sqrt{n}W^{(m)}_{1, P^{(m)}}}{\sigma_{P^{(m)}}^{(m)}}\frac{\sigma_{P^{(m)}}^{(m)}}{\sigma_{P^{(m)}}}+\frac{\sqrt{n}W^{(m)}_{2, P^{(m)}}}{\sigma_{P^{(m)}}} + \tau_\alpha- \tau_\alpha \frac{\hat{\sigma}^{(n,m)}}{\sigma_{P^{(m)}}^{(m)}}\frac{\sigma_{P^{(m)}}^{(m)}}{\sigma_{P^{(m)}}} \right)=\\
   &=\frac{\sqrt{n}W^{(m)}_{1, P^{(m)}}}{\sigma_{P^{(m)}}^{(m)}}\left(1-\frac{\sigma_{P^{(m)}}^{(m)}}{\sigma_{P^{(m)}}}\right)-\frac{\sqrt{n}W^{(m)}_{2, P^{(m)}}}{\sigma_{P^{(m)}}} + \tau_\alpha\left(\frac{\hat{\sigma}^{(n,m)}}{\sigma_{P^{(m)}}^{(m)}}-1\right)\left(\frac{\sigma_{P^{(m)}}^{(m)}}{\sigma_{P^{(m)}}}-1\right)+\tau_\alpha\left(\frac{\sigma_{P^{(m)}}^{(m)}}{\sigma_{P^{(m)}}}-1\right)+\tau_\alpha\left(\frac{\hat{\sigma}^{(n,m)}}{\sigma_{P^{(m)}}^{(m)}}-1\right)\\
   &= o_p(1) \text{ as }m\to \infty
\end{align*}

To see why the random quantity above converges to zero in probability, see that because of Assumption \ref{assump:assump3_stfr}, Lemma \ref{lemma:lemma1_stfr}, and continuous mapping theorem, we have that 
\[
\frac{\hat{\sigma}^{(n,m)}}{\sigma_{P^{(m)}}^{(m)}}-1= o_p(1) \text{ and }\frac{\sigma_{P^{(m)}}^{(m)}}{\sigma_{P^{(m)}}}-1= o_p(1) \text{ as }m\to \infty
\]
Additionally, because of Assumptions \ref{assump:assump1_stfr}, \ref{assump:assump3_stfr} and condition $n=o(m^{2\gamma})$, we have that
\[
\left|\frac{\sqrt{n}W^{(m)}_{2, P^{(m)}}}{\sigma_{P^{(m)}}}\right|=\left|\frac{o(m^{\gamma})\cO_p(m^{-\gamma})}{\sigma_{P^{(m)}}}\right|\leq \left|\frac{o(m^{\gamma})\cO_p(m^{-\gamma})}{\inf_{P\in\cP}\sigma_{P}}\right|=o_p(1)
\]

Finally, 
\begin{align*}
    &\frac{\sqrt{n}W^{(m)}_{1, P^{(m)}}}{\sigma_{P^{(m)}}^{(m)}}\frac{\sigma_{P^{(m)}}^{(m)}}{\sigma_{P^{(m)}}}+\frac{\sqrt{n}W^{(m)}_{2, P^{(m)}}}{\sigma_{P^{(m)}}} + \tau_\alpha- \tau_\alpha \frac{\hat{\sigma}^{(n,m)}}{\sigma_{P^{(m)}}^{(m)}}\frac{\sigma_{P^{(m)}}^{(m)}}{\sigma_{P^{(m)}}}=\\
    &=\frac{\sqrt{n}W^{(m)}_{1, P^{(m)}}}{\sigma_{P^{(m)}}^{(m)}} - \left[ \frac{\sqrt{n}W^{(m)}_{1, P^{(m)}}}{\sigma_{P^{(m)}}^{(m)}}- \left(\frac{\sqrt{n}W^{(m)}_{1, P^{(m)}}}{\sigma_{P^{(m)}}^{(m)}}\frac{\sigma_{P^{(m)}}^{(m)}}{\sigma_{P^{(m)}}}+\frac{\sqrt{n}W^{(m)}_{2, P^{(m)}}}{\sigma_{P^{(m)}}} + \tau_\alpha- \tau_\alpha \frac{\hat{\sigma}^{(n,m)}}{\sigma_{P^{(m)}}^{(m)}}\frac{\sigma_{P^{(m)}}^{(m)}}{\sigma_{P^{(m)}}} \right) \right]\\
    &=\frac{\sqrt{n}W^{(m)}_{1, P^{(m)}}}{\sigma_{P^{(m)}}^{(m)}} + o_p(1)\Rightarrow N(0,1)
\end{align*}

by Slutsky's theorem. Because $N(0,1)$ is a continuous distribution, we have uniform convergence of the distribution function \citep{resnick2019probability}[Chapter 8, Exercise 5] and we do not have to worry about the fact that $\tau_\alpha -\frac{\sqrt{n}\Omega_{P^{(m)}}^{\textup{STFR}}}{\sigma_{P^{(m)}}}$ depends on $m$.



\textit{Conditions to apply the central limit theorem.} Now, we comment on the conditions for the central limit theorem \citep[Corollary 9.5.11]{cappe2009inference}. Define our triangular array as $\left\{V^{(m)}_{i}\right\}_{1 \leq i \leq n}$, where
$V^{(m)}_{i}\triangleq \frac{T_i^{(m)}-\Ex_{P^{(m)}}[T_i^{(m)} \mid \cD_{tr}^{(m)}]}{\sigma_{P^{(m)}}^{(m)}}$. 
\begin{enumerate}
    \item This condition naturally applies by definition and because of Assumption \ref{assump:assump2_stfr}.

    \item  See that, for any $m$, we have that
    \[
    \Ex_{P^{(m)}}[(V^{(m)}_{i})^2 \mid \cD_{tr}^{(m)}]=1
    \]
    
    \item Fix any $\epsilon>0$ and let $k$ be defined as in Assumption \ref{assump:assump2_stfr}. See that
    \begin{align*}
        &\Ex_{P^{(m)}}\left[ (V^{(m)}_{i})^2\ones[|V^{(m)}_{i}|\geq \epsilon n] \mid  \cD_{tr}^{(m)}\right]= \\ 
        &= \Ex_{P^{(m)}}\left[(V^{(m)}_{i})^2 \ones[(|V^{(m)}_{i}|/(\epsilon n))^{k}\geq 1] \mid  \cD_{tr}^{(m)}\right]\\
        &\leq \frac{1}{(n\epsilon)^{k}} \Ex_{P^{(m)}}\left[|V^{(m)}_{i}|^{2+k}\mid  \cD_{tr}^{(m)}\right]\\
        &= \frac{1}{(n\epsilon)^{k}} \Ex_{P^{(m)}}\left[\left|\frac{T_i^{(m)}-\Ex_{P^{(m)}}[T_i^{(m)} \mid \cD_{tr}^{(m)}]}{\sigma_{P^{(m)}}^{(m)}}\right|^{2+k}\mid  \cD_{tr}^{(m)}\right]\\
        &\leq \frac{1}{(n\epsilon)^{k}} \frac{1}{(\sigma_{P^{(m)}}^{(m)})^{2+k}} \left\{\Ex_{P^{(m)}}\left[|T^{(m)}_i|^{2+k}\mid  \cD_{tr}^{(m)}\right]^{\frac{1}{2+k}} + \Ex_{P^{(m)}}\left[|T^{(m)}_i|\mid  \cD_{tr}^{(m)}\right] \right\}^{2+k}\\
        &= \frac{1}{(n\epsilon)^{k}} \left[\frac{1}{(\sigma_{P^{(m)}})^{2+k}} +o_p(1)\right]\left\{\Ex_{P^{(m)}}\left[|T^{(m)}_i|^{2+k}\mid  \cD_{tr}^{(m)}\right]^{\frac{1}{2+k}} + \Ex_{P^{(m)}}\left[|T^{(m)}_i|\mid  \cD_{tr}^{(m)}\right] \right\}^{2+k}\\
        &\leq \frac{1}{(n\epsilon)^{k}} \left[\frac{1}{(\inf_{P\in \cP}\sigma_{P})^{2+k}} +o_p(1)\right]\cO_p(1)\\
        &= \frac{1}{(n\epsilon)^{k}} \cO_p(1)\\
        &= o_p(1)
    \end{align*}
    where the third inequality is obtained via Minkowski Inequality \citep{resnick2019probability} and the last inequality is an application of Assumption \ref{assump:assump2_stfr} and \citet[Example 6.5.2]{resnick2019probability}.
\end{enumerate}
\end{proof}

\textbf{Corollary \ref{cor:cor1_stfr}}. Suppose we are under the conditions of Theorem \ref{thm:thm1_stfr}.

$\bullet$ (Type-I error) If $H_0:X\indep Y\mid Z$ holds, then
\begin{align*}
            & \Ex_P[\varphi^{\textup{STFR}}_\alpha(\cD^{(n)}_{te},\cD_{tr}^{(m)})]\leq 1-\Phi\left(\tau_{\alpha}-\sqrt{\frac{n}{\sigma_P^2}}\Delta_{2,P}\right) +o(1)
\end{align*}
where $o(1)$ denotes uniform convergence over all $P \in \cP_0$ as $m\to \infty$.

$\bullet$ (Type-II error) In general, we have
\begin{align*}
        &1-\Ex_P[\varphi^{\textup{STFR}}_\alpha(\cD^{(n)}_{te},\cD_{tr}^{(m)})]\leq\Phi\left(\tau_{\alpha}-\sqrt{\frac{n}{\sigma_P^2}}(\Delta_P-\Delta_{1,P})\right) +o(1)
\end{align*}
where $o(1)$ denotes uniform convergence over all $P \in \cP$ as $m\to \infty$ and $\Delta_P \triangleq  \Ex_P [\ell (f^*_{2,P}(Z),Y)]- \Ex_P [\ell (f^*_{1,P}(X,Z),Y)]$.

\begin{proof}

Under the conditions of Theorem \ref{thm:thm1_stfr}, we start proving that
    \begin{enumerate}
         \item $\Delta_P-\Delta_{1,P} \leq \Omega_P^{\textup{STFR}}$ holds;
        \item Under $H_0$, $\Omega_P^{\textup{STFR}} \leq \Delta_{2,P}$ holds. 
    \end{enumerate}
     For (1), see that,
\begin{align*}
    \Omega_P^{\textup{STFR}}&=\Ex_P[\ell(g_{2,P}^*(Z),Y)]-\Ex_P[\ell(g_{1,P}^*(X,Z),Y)]\\
    &=\Ex_P[\ell(g_{2,P}^*(Z),Y)]-\Ex_P[\ell(f_{2,P}^*(Z),Y)]~~~~~~~~~~~~~~~(\geq 0)\\
    &+\Ex_P[\ell(f_{1,P}^*(X,Z),Y)]-\Ex_P[\ell(g_{1,P}^*(X,Z),Y)]\\
    &+\Ex_P[\ell(f_{2,P}^*(Z),Y)]-\Ex_P[\ell(f_{1,P}^*(X,Z),Y)]\\
    &\geq \Ex_P[\ell(f_{1,P}^*(X,Z),Y)]-\Ex_P[\ell(g_{1,P}^*(X,Z),Y)]+\Delta_P\\
    &= \Delta_P-\Delta_{1,P}
\end{align*}


Now, for (2):
\begin{align*}
\Omega_P^{\textup{STFR}}&=\Ex_P[\ell(g_{2,P}^*(Z),Y)]-\Ex_P[\ell(g_{1,P}^*(X,Z),Y)]\\
    &=\Ex_P[\ell(g_{2,P}^*(Z),Y)]-\Ex_P[\ell(f_{2,P}^*(Z),Y)]\\
    &+\Ex_P[\ell(f_{1,P}^*(X,Z),Y)]-\Ex_P[\ell(g_{1,P}^*(X,Z),Y)]~~~~~~~~~~(\leq 0)\\
    &+\Ex_P[\ell(f_{2,P}^*(Z),Y)]-\Ex_P[\ell(f_{1,P}^*(X,Z),Y)] ~~~~~~~~~~~~~~~(= 0\text{, because $H_0$ holds})\\
    &\leq  \Ex_P[\ell(g_{2,P}^*(Z),Y)]-\Ex_P[\ell(f_{2,P}^*(Z),Y)]\\
    &=\Delta_{2,P}
\end{align*}

Finally, see that

\[
1-\Phi\left(\tau_{\alpha}-\sqrt{\frac{n}{\sigma_P^2}}\Omega_P^{\textup{STFR}}\right)\leq 1-\Phi\left(\tau_{\alpha}-\sqrt{\frac{n}{\sigma_P^2}}\Delta_{2,P}\right)
\]
and
$$\Phi\left(\tau_{\alpha}-\sqrt{\frac{n}{\sigma_P^2}}\Omega_P^{\textup{STFR}}\right)\leq \Phi\left(\tau_{\alpha}-\sqrt{\frac{n}{\sigma_P^2}}(\Delta_P-\Delta_{1,P})\right)$$
Combining these observations with Theorem \ref{thm:thm1_stfr}, we get the result.
\end{proof}



    

\subsection{GCM }

\textbf{Theorem \ref{thm:thm1_gcm}}. Suppose that Assumptions \ref{assump:assump1_gcm}, \ref{assump:assump2_stfr}, and \ref{assump:assump3_stfr} hold. If $n$ is a function of $m$ such that $n\to \infty$ and $n=o(m^{\gamma})$ as $m\to \infty$,  then
\begin{align*}
    \Ex_P[\varphi^{\textup{GCM}}_\alpha(\cD^{(n)}_{te}, \cD^{(m)}_{tr})]&= 1-\Phi\left(\tau_{\alpha/2}-\sqrt{\frac{n}{\sigma_P^2}}\Omega_P^{\textup{GCM}}\right)+\Phi\left(-\tau_{\alpha/2}-\sqrt{\frac{n}{\sigma_P^2}}\Omega_P^{\textup{GCM}}\right)+o(1)
\end{align*}
where $o(1)$ denotes uniform convergence over all $P \in \cP$ as $m\to \infty$ and
\[
\Omega_P^{\textup{GCM}}\triangleq\Ex_P[\Cov_P(X,Y\mid Z)]+\Ex_P[\delta_{1,P}(Z)\delta_{2,P}(Z)]
\]
\begin{proof}
First, note that there must be\footnote{Because of the definition of $\sup$.} a sequence of probability measures in $\cP$, $(P^{(m)})_{m\in\mathbb{N}}$, such that
\begin{align*}
   &\sup_{P\in \cP}\left|\Ex_P[\varphi^{\textup{GCM}}_\alpha(\cD^{(n)}_{te},\cD_{tr}^{(m)})] -1+\Phi\left(\tau_{\alpha/2}-\sqrt{\frac{n}{\sigma_P^2}}\Omega_P^{\textup{GCM}}\right)-\Phi\left(-\tau_{\alpha/2}-\sqrt{\frac{n}{\sigma_P^2}}\Omega_P^{\textup{GCM}}\right)\right|\leq\\&\leq \left|\Ex_{P^{(m)}}[\varphi^{\textup{GCM}}_\alpha(\cD^{(n)}_{te},\cD_{tr}^{(m)})] -1+\Phi\left(\tau_{\alpha/2}-\sqrt{\frac{n}{\sigma_{P^{(m)}}^2}}\Omega_{P^{(m)}}^{\textup{GCM}}\right)-\Phi\left(-\tau_{\alpha/2}-\sqrt{\frac{n}{\sigma_{P^{(m)}}^2}}\Omega_{P^{(m)}}^{\textup{GCM}}\right)\right| + \frac{1}{m}
\end{align*}

Then, it suffices to show that the RHS vanishes when we consider such a sequence $(P^{(m)})_{m\in\mathbb{N}}$.

Now, let us first decompose the test statistic $\Gamma^{(n,m)}$ in the following way:
\begin{align*}
        &\Gamma^{(n,m)}\triangleq\Bigg|\frac{\sqrt{n}\bar{T}^{(n,m)}}{\hat{\sigma}^{(n,m)}}\Bigg|=\\
        &=\Bigg|\frac{\sqrt{n}\Big(\bar{T}^{(n,m)}-\Ex_{P^{(m)}}[T^{(m)}_1\mid \cD_{tr}^{(m)}]\Big)}{\hat{\sigma}^{(n,m)}}+\frac{\sqrt{n}\Ex_{P^{(m)}}[T^{(m)}_1\mid \cD_{tr}^{(m)}]}{\hat{\sigma}^{(n,m)}}\Bigg|\\
        &=\Bigg|\frac{\sqrt{n}\Big(\bar{T}^{(n,m)}-\Ex_{P^{(m)}}[T^{(m)}_1\mid \cD_{tr}^{(m)}]\Big)}{\hat{\sigma}^{(n,m)}}+ \frac{\sqrt{n}\Ex_{P^{(m)}}[(\hat{g}^{(m)}_{1}(Z_1)-g^{*}_{1,P^{(m)}}(Z_1))(\hat{g}^{(m)}_{2}(Z_1)-g^{*}_{2,P^{(m)}}(Z_1))\mid \cD_{tr}^{(m)}]}{\hat{\sigma}^{(n,m)}}\\
        &+ \frac{\sqrt{n}\Ex_{P^{(m)}}[(\hat{g}^{(m)}_{1}(Z_1)-g^{*}_{1,P^{(m)}}(Z_1))\delta_{2,P^{(m)}}(Z_1)\mid \cD_{tr}^{(m)}]}{\hat{\sigma}^{(n,m)}}+\frac{\sqrt{n}\Ex_{P^{(m)}}[\delta_{1,P^{(m)}}(Z_1)(\hat{g}^{(m)}_{2}(Z_1)-g^{*}_{2,P^{(m)}}(Z_1))\mid \cD_{tr}^{(m)}]}{\hat{\sigma}^{(n,m)}}\\
        &+ \frac{\sqrt{n}\Omega_{P^{(m)}}^{\textup{GCM}}}{\hat{\sigma}^{(n,m)}}\Bigg|\\
        &=\Bigg| \frac{\sqrt{n}W^{(m)}_{1, P^{(m)}}}{\hat{\sigma}^{(n,m)}}+\frac{\sqrt{n}W^{(m)}_{2, P^{(m)}}}{\hat{\sigma}^{(n,m)}} + \frac{\sqrt{n}W^{(m)}_{3, P^{(m)}}}{\hat{\sigma}^{(n,m)}}+\frac{\sqrt{n}W^{(m)}_{4, P^{(m)}}}{\hat{\sigma}^{(n,m)}} + \frac{\sqrt{n}\Omega_{P^{(m)}}^{\textup{GCM}}}{\hat{\sigma}^{(n,m)}}\Bigg|
\end{align*}

The terms involving one of the $\epsilon$ and $\eta$ were all zero and were omitted. Given that $n$ is a function of $m$, we omit it when writing the $W^{(m)}_{j,P^{(m)}}$'s. Define $\sigma_{P^{(m)}}^{(m)}\triangleq \sqrt{\Var_{P^{(m)}}[T^{(m)}_1\mid  \cD_{tr}^{(m)}]}$ and see that
\begin{align}
    &\Ex_P[\varphi^{\textup{GCM}}_\alpha(\cD^{(n)}_{te},\cD_{tr}^{(m)})]= \nonumber\\
    &=\Pr_P[p(\cD^{(n)}_{te},\cD_{tr}^{(m)})\leq \alpha] \nonumber\\
    &=\Pr_P\left[1-\Phi\left(\Gamma^{(n,m)}\right)\leq \alpha/2 \right] \nonumber\\
    &=\Pr_P\left[\Gamma^{(n,m)} \geq \tau_{\alpha/2} \right] \nonumber\\
    &=\Pr_P\left[\frac{\sqrt{n}W^{(m)}_{1, P^{(m)}}}{\hat{\sigma}^{(n,m)}}+\frac{\sqrt{n}W^{(m)}_{2, P^{(m)}}}{\hat{\sigma}^{(n,m)}} + \frac{\sqrt{n}W^{(m)}_{3, P^{(m)}}}{\hat{\sigma}^{(n,m)}}+\frac{\sqrt{n}W^{(m)}_{4, P^{(m)}}}{\hat{\sigma}^{(n,m)}} + \frac{\sqrt{n}\Omega_{P^{(m)}}^{\textup{GCM}}}{\hat{\sigma}^{(n,m)}} \leq -\tau_{\alpha/2} \right] + \nonumber\\
    &~~~ +\Pr_P\left[\frac{\sqrt{n}W^{(m)}_{1, P^{(m)}}}{\hat{\sigma}^{(n,m)}}+\frac{\sqrt{n}W^{(m)}_{2, P^{(m)}}}{\hat{\sigma}^{(n,m)}} + \frac{\sqrt{n}W^{(m)}_{3, P^{(m)}}}{\hat{\sigma}^{(n,m)}}+\frac{\sqrt{n}W^{(m)}_{4, P^{(m)}}}{\hat{\sigma}^{(n,m)}} + \frac{\sqrt{n}\Omega_{P^{(m)}}^{\textup{GCM}}}{\hat{\sigma}^{(n,m)}} \geq \tau_{\alpha/2} \right] \nonumber\\
    &=\Pr_P\left[\frac{\sqrt{n}W^{(m)}_{1, P^{(m)}}}{\sigma^{(m)}_{P^{(m)}}}\frac{\sigma^{(m)}_{P^{(m)}}}{\sigma_{P^{(m)}}}+\frac{\sqrt{n}W^{(m)}_{2, P^{(m)}}}{\sigma_{P^{(m)}}} + \frac{\sqrt{n}W^{(m)}_{3, P^{(m)}}}{\sigma_{P^{(m)}}}+\frac{\sqrt{n}W^{(m)}_{4, P^{(m)}}}{\sigma_{P^{(m)}}}  +\frac{\hat{\sigma}^{(n,m)}}{\sigma^{(m)}_{P^{(m)}}}\frac{\sigma^{(m)}_{P^{(m)}}}{\sigma_{P^{(m)}}}\tau_{\alpha/2}-\tau_{\alpha/2} \leq -\tau_{\alpha/2} -  \frac{\sqrt{n}\Omega_{P^{(m)}}^{\textup{GCM}}}{\sigma_{P^{(m)}}} \right] + \nonumber\\
    &~~~ +\Pr_P\left[\frac{\sqrt{n}W^{(m)}_{1, P^{(m)}}}{\sigma^{(m)}_{P^{(m)}}}\frac{\sigma^{(m)}_{P^{(m)}}}{\sigma_{P^{(m)}}}+\frac{\sqrt{n}W^{(m)}_{2, P^{(m)}}}{\sigma_{P^{(m)}}} + \frac{\sqrt{n}W^{(m)}_{3, P^{(m)}}}{\sigma_{P^{(m)}}}+\frac{\sqrt{n}W^{(m)}_{4, P^{(m)}}}{\sigma_{P^{(m)}}}  -\frac{\hat{\sigma}^{(n,m)}}{\sigma^{(m)}_{P^{(m)}}}\frac{\sigma^{(m)}_{P^{(m)}}}{\sigma_{P^{(m)}}}\tau_{\alpha/2}+\tau_{\alpha/2} \geq \tau_{\alpha/2} -  \frac{\sqrt{n}\Omega_{P^{(m)}}^{\textup{GCM}}}{\sigma_{P^{(m)}}} \right] \nonumber\\
    %&=\Pr_P\left[\frac{\sqrt{n}W^{(m)}_{1, P^{(m)}}}{\sigma^{(m)}_{P^{(m)}}} \leq -\tau_{\alpha/2} -  \frac{\sqrt{n}\Omega_{P^{(m)}}^{\textup{GCM}}}{\sigma_{P^{(m)}}} \right]  +\Pr_P\left[\frac{\sqrt{n}W^{(m)}_{1, P^{(m)}}}{\sigma^{(m)}_{P^{(m)}}} \geq \tau_{\alpha/2} -  \frac{\sqrt{n}\Omega_{P^{(m)}}^{\textup{GCM}}}{\sigma_{P^{(m)}}} \right] +o(1) \label{step:step1_gcm}\\
    &=1-\Phi\left(\tau_{\alpha/2}-\sqrt{\frac{n}{\sigma_{P^{(m)}}^2}}\Omega_{P^{(m)}}^{\textup{GCM}}\right)+\Phi\left(-\tau_{\alpha/2}-\sqrt{\frac{n}{\sigma_{P^{(m)}}^2}}\Omega_{P^{(m)}}^{\textup{GCM}}\right)+o(1) \label{step:step1_gcm}
\end{align}

Implying that
\begin{align*}
   &\sup_{P\in \cP}\left|\Ex_P[\varphi^{\textup{GCM}}_\alpha(\cD^{(n)}_{te},\cD_{tr}^{(m)})] -1+\Phi\left(\tau_{\alpha/2}-\sqrt{\frac{n}{\sigma_P^2}}\Omega_P^{\textup{GCM}}\right)-\Phi\left(-\tau_{\alpha/2}-\sqrt{\frac{n}{\sigma_P^2}}\Omega_P^{\textup{GCM}}\right)\right|= o(1) \text{ as }m\to \infty
\end{align*}


\textit{Justifying step \ref{step:step1_gcm}.} First, from a central limit theorem for triangular arrays \citep[Corollary 9.5.11]{cappe2009inference}, we have that
\[
\sqrt{n}\left(\frac{W^{(m)}_{1, P^{(m)}}}{\sigma_{P^{(m)}}^{(m)}}\right)= \sqrt{n}\left(\frac{\bar{T}^{(n,m)}-\Ex_{P^{(m)}}[T^{(m)}_1 \mid \cD_{tr}^{(m)}]}{\sigma_{P^{(m)}}^{(m)}}\right) = \frac{1}{\sqrt{n}}\sum_{i=1}^n\left(\frac{T_i^{(m)}-\Ex_{P^{(m)}}[T^{(m)}_1 \mid \cD_{tr}^{(m)}]}{\sigma_{P^{(m)}}^{(m)}}\right)\Rightarrow N(0,1)
\]
The conditions for the central limit theorem \citep[Corollary 9.5.11]{cappe2009inference} can be proven to hold like in Theorem \ref{thm:thm1_stfr}'s proof.

Second, we have that
\begin{align*}
   &\frac{\sqrt{n}W^{(m)}_{1, P^{(m)}}}{\sigma_{P^{(m)}}^{(m)}}- \left(\frac{\sqrt{n}W^{(m)}_{1, P^{(m)}}}{\sigma_{P^{(m)}}^{(m)}}\frac{\sigma_{P^{(m)}}^{(m)}}{\sigma_{P^{(m)}}}+\frac{\sqrt{n}W^{(m)}_{2, P^{(m)}}}{\sigma_{P^{(m)}}} + \frac{\sqrt{n}W^{(m)}_{3, P^{(m)}}}{\sigma_{P^{(m)}}}+\frac{\sqrt{n}W^{(m)}_{4, P^{(m)}}}{\sigma_{P^{(m)}}}- \tau_{\alpha/2}+ \tau_{\alpha/2} \frac{\hat{\sigma}^{(n,m)}}{\sigma_{P^{(m)}}^{(m)}}\frac{\sigma_{P^{(m)}}^{(m)}}{\sigma_{P^{(m)}}} \right)=\\
   &=\frac{\sqrt{n}W^{(m)}_{1, P^{(m)}}}{\sigma_{P^{(m)}}^{(m)}}\left(1-\frac{\sigma_{P^{(m)}}^{(m)}}{\sigma_{P^{(m)}}}\right)-\frac{\sqrt{n}W^{(m)}_{2, P^{(m)}}}{\sigma_{P^{(m)}}} - \frac{\sqrt{n}W^{(m)}_{3, P^{(m)}}}{\sigma_{P^{(m)}}}-\frac{\sqrt{n}W^{(m)}_{4, P^{(m)}}}{\sigma_{P^{(m)}}}+\\
   &~~~~~ + \tau_{\alpha/2}\left(1-\frac{\hat{\sigma}^{(n,m)}}{\sigma_{P^{(m)}}^{(m)}}\right)\left(\frac{\sigma_{P^{(m)}}^{(m)}}{\sigma_{P^{(m)}}}-1\right)+\tau_{\alpha/2}\left(1-\frac{\sigma_{P^{(m)}}^{(m)}}{\sigma_{P^{(m)}}}\right)+\tau_{\alpha/2}\left(1-\frac{\hat{\sigma}^{(n,m)}}{\sigma_{P^{(m)}}^{(m)}}\right)\\
   &= o_p(1) \text{ as }m\to \infty
\end{align*}

and 

\begin{align*}
   &\frac{\sqrt{n}W^{(m)}_{1, P^{(m)}}}{\sigma_{P^{(m)}}^{(m)}}- \left(\frac{\sqrt{n}W^{(m)}_{1, P^{(m)}}}{\sigma_{P^{(m)}}^{(m)}}\frac{\sigma_{P^{(m)}}^{(m)}}{\sigma_{P^{(m)}}}+\frac{\sqrt{n}W^{(m)}_{2, P^{(m)}}}{\sigma_{P^{(m)}}} + \frac{\sqrt{n}W^{(m)}_{3, P^{(m)}}}{\sigma_{P^{(m)}}}+\frac{\sqrt{n}W^{(m)}_{4, P^{(m)}}}{\sigma_{P^{(m)}}}+ \tau_{\alpha/2}- \tau_{\alpha/2} \frac{\hat{\sigma}^{(n,m)}}{\sigma_{P^{(m)}}^{(m)}}\frac{\sigma_{P^{(m)}}^{(m)}}{\sigma_{P^{(m)}}} \right)=\\
   &=\frac{\sqrt{n}W^{(m)}_{1, P^{(m)}}}{\sigma_{P^{(m)}}^{(m)}}\left(1-\frac{\sigma_{P^{(m)}}^{(m)}}{\sigma_{P^{(m)}}}\right)-\frac{\sqrt{n}W^{(m)}_{2, P^{(m)}}}{\sigma_{P^{(m)}}} - \frac{\sqrt{n}W^{(m)}_{3, P^{(m)}}}{\sigma_{P^{(m)}}}-\frac{\sqrt{n}W^{(m)}_{4, P^{(m)}}}{\sigma_{P^{(m)}}}+\\
   &~~~~~ + 
   \tau_{\alpha/2}\left(\frac{\hat{\sigma}^{(n,m)}}{\sigma_{P^{(m)}}^{(m)}}-1\right)\left(\frac{\sigma_{P^{(m)}}^{(m)}}{\sigma_{P^{(m)}}}-1\right)+\tau_{\alpha/2}\left(\frac{\sigma_{P^{(m)}}^{(m)}}{\sigma_{P^{(m)}}}-1\right)+\tau_{\alpha/2}\left(\frac{\hat{\sigma}^{(n,m)}}{\sigma_{P^{(m)}}^{(m)}}-1\right)\\
   &= o_p(1) \text{ as }m\to \infty
\end{align*}

To see why the random quantities above converge to zero in probability, see that because of Assumption \ref{assump:assump3_stfr}, Lemma\footnote{We can apply this STFR's lemma because it still holds when we consider GCM's test statistic.} \ref{lemma:lemma1_stfr}, and continuous mapping theorem, we have that 
\[
\frac{\hat{\sigma}^{(n,m)}}{\sigma_{P^{(m)}}^{(m)}}-1= o_p(1) \text{ and }\frac{\sigma_{P^{(m)}}^{(m)}}{\sigma_{P^{(m)}}}-1= o_p(1) \text{ as }m\to \infty
\]
Additionally, because of Assumptions \ref{assump:assump1_gcm}, \ref{assump:assump3_stfr}, Cauchy-Schwarz inequality, and condition $n=o(m^{\gamma})$, we have that
\begin{align*}
        &\left|\frac{\sqrt{n}W^{(m)}_{2, P^{(m)}}}{\sigma_{P^{(m)}}}\right|=\left|\frac{\sqrt{n}\Ex_{P^{(m)}}[(\hat{g}^{(m)}_{1}(Z_1)-g^{*}_{1,P^{(m)}}(Z_1))(\hat{g}^{(m)}_{2}(Z_1)-g^{*}_{2,P^{(m)}}(Z_1))\mid \cD_{tr}^{(m)}]}{\sigma_{P^{(m)}}}\right|\\
        &\leq  \frac{\sqrt{n\Ex_{P^{(m)}}[(\hat{g}^{(m)}_{1}(Z_1)-g^{*}_{1,P^{(m)}}(Z_1))^2\mid \cD_{tr}^{(m)}]\Ex_{P^{(m)}}[(\hat{g}^{(m)}_{2}(Z_1)-g^{*}_{2,P^{(m)}}(Z_1))^2\mid \cD_{tr}^{(m)}]}}{\inf_{P\in\cP}\sigma_{P}}\\
        &=\frac{\sqrt{o(m^{\gamma})\cO_p(m^{-2\gamma})}}{\inf_{P\in\cP}\sigma_{P}}\\
        &=o_p(1)
\end{align*}
\begin{align*}
        &\left|\frac{\sqrt{n}W^{(m)}_{3, P^{(m)}}}{\sigma_{P^{(m)}}}\right|=\left|\frac{\sqrt{n}\Ex_{P^{(m)}}[(\hat{g}^{(m)}_{1}(Z_1)-g^{*}_{1,P^{(m)}}(Z_1))\delta_{2,P^{(m)}}(Z_1)\mid \cD_{tr}^{(m)}]}{\sigma_{P^{(m)}}}\right|\\
        &\leq  \frac{\sqrt{n\Ex_{P^{(m)}}[(\hat{g}^{(m)}_{1}(Z_1)-g^{*}_{1,P^{(m)}}(Z_1))^2\mid \cD_{tr}^{(m)}]\Ex_{P^{(m)}}[(\delta_{2,P^{(m)}}(Z_1))^2]}}{\inf_{P\in\cP}\sigma_{P}}\\
        &=\frac{\sqrt{o(m^{\gamma})\cO_p(m^{-\gamma})}}{\inf_{P\in\cP}\sigma_{P}}\\
        &=o_p(1)
\end{align*}
\begin{align*}
        &\left|\frac{\sqrt{n}W^{(m)}_{4, P^{(m)}}}{\sigma_{P^{(m)}}}\right|=\left|\frac{\sqrt{n}\Ex_{P^{(m)}}[(\hat{g}^{(m)}_{2}(Z_1)-g^{*}_{2,P^{(m)}}(Z_1))\delta_{1,P^{(m)}}(Z_1)\mid \cD_{tr}^{(m)}]}{\sigma_{P^{(m)}}}\right|\\
        &\leq  \frac{\sqrt{n\Ex_{P^{(m)}}[(\hat{g}^{(m)}_{2}(Z_1)-g^{*}_{2,P^{(m)}}(Z_1))^2\mid \cD_{tr}^{(m)}]\Ex_{P^{(m)}}[(\delta_{1,P^{(m)}}(Z_1))^2]}}{\inf_{P\in\cP}\sigma_{P}}\\
        &=\frac{\sqrt{o(m^{\gamma})\cO_p(m^{-\gamma})}}{\inf_{P\in\cP}\sigma_{P}}\\
        &=o_p(1)
\end{align*}

Finally, 
\begin{align*}
    &\left(\frac{\sqrt{n}W^{(m)}_{1, P^{(m)}}}{\sigma_{P^{(m)}}^{(m)}}\frac{\sigma_{P^{(m)}}^{(m)}}{\sigma_{P^{(m)}}}+\frac{\sqrt{n}W^{(m)}_{2, P^{(m)}}}{\sigma_{P^{(m)}}} + \frac{\sqrt{n}W^{(m)}_{3, P^{(m)}}}{\sigma_{P^{(m)}}}+\frac{\sqrt{n}W^{(m)}_{4, P^{(m)}}}{\sigma_{P^{(m)}}}- \tau_{\alpha/2}+ \tau_{\alpha/2} \frac{\hat{\sigma}^{(n,m)}}{\sigma_{P^{(m)}}^{(m)}}\frac{\sigma_{P^{(m)}}^{(m)}}{\sigma_{P^{(m)}}} \right)=\\
    &=\frac{\sqrt{n}W^{(m)}_{1, P^{(m)}}}{\sigma_{P^{(m)}}^{(m)}} - \left[\frac{\sqrt{n}W^{(m)}_{1, P^{(m)}}}{\sigma_{P^{(m)}}^{(m)}}- \left(\frac{\sqrt{n}W^{(m)}_{1, P^{(m)}}}{\sigma_{P^{(m)}}^{(m)}}\frac{\sigma_{P^{(m)}}^{(m)}}{\sigma_{P^{(m)}}}+\frac{\sqrt{n}W^{(m)}_{2, P^{(m)}}}{\sigma_{P^{(m)}}} + \frac{\sqrt{n}W^{(m)}_{3, P^{(m)}}}{\sigma_{P^{(m)}}}+\frac{\sqrt{n}W^{(m)}_{4, P^{(m)}}}{\sigma_{P^{(m)}}}- \tau_{\alpha/2}+ \tau_{\alpha/2} \frac{\hat{\sigma}^{(n,m)}}{\sigma_{P^{(m)}}} \right) \right]\\
    &=\frac{\sqrt{n}W^{(m)}_{1, P^{(m)}}}{\sigma_{P^{(m)}}^{(m)}} + o_p(1)\Rightarrow N(0,1)
\end{align*}

and 
\begin{align*}
    & \left(\frac{\sqrt{n}W^{(m)}_{1, P^{(m)}}}{\sigma_{P^{(m)}}^{(m)}}\frac{\sigma_{P^{(m)}}^{(m)}}{\sigma_{P^{(m)}}}+\frac{\sqrt{n}W^{(m)}_{2, P^{(m)}}}{\sigma_{P^{(m)}}} + \frac{\sqrt{n}W^{(m)}_{3, P^{(m)}}}{\sigma_{P^{(m)}}}+\frac{\sqrt{n}W^{(m)}_{4, P^{(m)}}}{\sigma_{P^{(m)}}}+ \tau_{\alpha/2}- \tau_{\alpha/2} \frac{\hat{\sigma}^{(n,m)}}{\sigma_{P^{(m)}}^{(m)}}\frac{\sigma_{P^{(m)}}^{(m)}}{\sigma_{P^{(m)}}} \right)=\\
    &=\frac{\sqrt{n}W^{(m)}_{1, P^{(m)}}}{\sigma_{P^{(m)}}^{(m)}} - \left[\frac{\sqrt{n}W^{(m)}_{1, P^{(m)}}}{\sigma_{P^{(m)}}^{(m)}}- \left(\frac{\sqrt{n}W^{(m)}_{1, P^{(m)}}}{\sigma_{P^{(m)}}^{(m)}}\frac{\sigma_{P^{(m)}}^{(m)}}{\sigma_{P^{(m)}}}+\frac{\sqrt{n}W^{(m)}_{2, P^{(m)}}}{\sigma_{P^{(m)}}} + \frac{\sqrt{n}W^{(m)}_{3, P^{(m)}}}{\sigma_{P^{(m)}}}+\frac{\sqrt{n}W^{(m)}_{4, P^{(m)}}}{\sigma_{P^{(m)}}}+ \tau_{\alpha/2}- \tau_{\alpha/2} \frac{\hat{\sigma}^{(n,m)}}{\sigma_{P^{(m)}}} \right) \right]\\
    &=\frac{\sqrt{n}W^{(m)}_{1, P^{(m)}}}{\sigma_{P^{(m)}}^{(m)}} + o_p(1)\Rightarrow N(0,1)
\end{align*}

by Slutsky's theorem. Because $N(0,1)$ is a continuous distribution, we have uniform convergence of the distribution function \citep{resnick2019probability}[Chapter 8, Exercise 5] and we do not have to worry about the fact that $\tau_{\alpha/2}-\sqrt{\frac{n}{\sigma_{P^{(m)}}^2}}\Omega_{P^{(m)}}^{\textup{GCM}}$ or $-\tau_{\alpha/2}-\sqrt{\frac{n}{\sigma_{P^{(m)}}^2}}\Omega_{P^{(m)}}^{\textup{GCM}}$ depends on $m$.

\end{proof}


\subsection{RESIT }

%p. 150 (https://link.springer.com/content/pdf/10.1007/978-0-8176-8409-9.pdf)

\begin{lemma}\label{lemma:lemma1_resit}
     Let $P_{U,V}$ and $P'_{U,V}$ be two distributions on $\big(\cU\times \cV, \cB(\cU\times \cV)\big)$, $\cU\times \cV\subseteq\reals^{d_U \times d_V}$, with $d_U, d_V\geq 1$. Assume $P_{U}$ and $P'_{U}$ are dominated by a common $\sigma$-finite measure $\mu$ and that $P_{V\mid U=u}=P'_{V\mid U=u}$ is dominated by a $\sigma$-finite measure $\nu_u$, for all $u \in \reals^{d_U}$. Then, 
     \[
     d_{\textup{TV}}(P_{U,V},P'_{U,V})=d_{\textup{TV}}(P_{U},P'_{U})
     \]
     where $d_\text{TV}$ denotes the total variation distance between two probability measures.
     \begin{proof}
     Let $p_U$ and $p'_U$ denote the densities of $P_{U}$ and $P'_{U}$ w.r.t. $\mu$, and let $p_{V|U}(\cdot \mid u)$ denote the density of $P_{V\mid U=u}=P'_{V\mid U=u}$ w.r.t. $\nu_u$. From Scheffe's theorem \citep{tsybakov2004introduction2}[Lemma 2.1], we have that:
     \begin{align*}
        d_{\textup{TV}}(P_{U,V},P'_{U,V})&=\frac{1}{2}\int \int |  p_U(u)p_{V|U}(v\mid u)-p'_U(u)p_{V|U}(v\mid u)| d\nu_u(v)d\mu(u)\\
        &=\frac{1}{2}\int  \left(\int |p_{V|U}(v\mid u)| d\nu_u(v)\right) | p_U(u) -p'_U(u)| d\mu(u)\\
        &=\frac{1}{2}\int  \left(\int p_{V|U}(v\mid u) d\nu_u(v)\right) | p_U(u) -p'_U(u)| d\mu(u)\\
        &=\frac{1}{2}\int | p_U(u) -p'_U(u)| d\mu(u)\\
        &=d_{\textup{TV}}(P_{U},P'_{U})
     \end{align*}
     \end{proof}
\end{lemma}

\begin{lemma}\label{lemma:lemma2_resit}
    For all $i\in[n]$, consider
    \[
        (\hat{\epsilon}_i,\hat{\eta}_i)\mid \cD^{(m)}_{tr} \sim P_{\hat{\epsilon},\hat{\eta}\mid \cD^{(m)}_{tr}},~~(\epsilon_i,\hat{\eta}_i)\mid \cD^{(m)}_{tr}\sim P_{\epsilon,\hat{\eta}\mid \cD^{(m)}_{tr}},~~(\hat{\epsilon}_i,\eta_i)\mid \cD^{(m)}_{tr} \sim P_{\hat{\epsilon},\eta\mid \cD^{(m)}_{tr}},
    \]
    where $\hat{\epsilon}_i=\epsilon_i -\delta_{1,P}(Z_i) - \left(\hat{g}^{(m)}_{1}(Z_i)-g^*_{1,P}(Z_i)\right)$ and $\hat{\eta}_i=\eta_i -\delta_{2,P}(Z_i) - \left(\hat{g}^{(m)}_{2}(Z_i)-g^*_{2,P}(Z_i)\right)$.

    Under Assumption \ref{assump:assump2_resit}  and $H_0:X\indep Y\mid Z$, we have that
    \begin{align*}
    \Ex_P[\varphi^{\textup{RESIT}}_\alpha(\cD^{(n)}_{te}, \cD^{(m)}_{tr}) \mid \cD^{(m)}_{tr}]\leq \alpha + \min \left\{d_{\textup{TV}}\left(P_{\hat{\epsilon},\hat{\eta}\mid \cD^{(m)}_{tr}}^n,P_{\epsilon,\hat{\eta}\mid \cD^{(m)}_{tr}}^n\right),d_{\textup{TV}}\left(P_{\hat{\epsilon},\hat{\eta}\mid \cD^{(m)}_{tr}}^n,P_{\hat{\epsilon},\eta\mid \cD^{(m)}_{tr}}^n\right)\right\}
    \end{align*}
    where $d_\text{TV}$ denotes the total variation distance between two probability measures.
\begin{proof}
    
Let us represent the stacked residuals (in matrix form) as $(\boldsymbol{\hat{\epsilon}},\boldsymbol{\hat{\eta}})=\{(\hat{\epsilon}_i,\hat{\eta}_i)\}_{i=1}^n$. See that 
\[
\bigg((\boldsymbol{\hat{\epsilon}},\boldsymbol{\hat{\eta}})^{(1)},\cdots,(\boldsymbol{\hat{\epsilon}},\boldsymbol{\hat{\eta}})^{(B)}\mid  (\boldsymbol{\hat{\epsilon}},\boldsymbol{\hat{\eta}})=(\boldsymbol{\bar{\epsilon}},\boldsymbol{\bar{\eta}}), \cD^{(m)}_{tr}\bigg)\overset{d}{=}\bigg((\boldsymbol{\epsilon},\boldsymbol{\hat{\eta}})^{(1)},\cdots,(\boldsymbol{\epsilon},\boldsymbol{\hat{\eta}})^{(B)}\mid  (\boldsymbol{\epsilon},\boldsymbol{\hat{\eta}})=(\boldsymbol{\bar{\epsilon}},\boldsymbol{\bar{\eta}}), \cD^{(m)}_{tr}\bigg)
\]
Then, because the random quantities above are conditionally discrete, their distribution is dominated by a counting measure depending on $(\boldsymbol{\bar{\epsilon}},\boldsymbol{\bar{\eta}})$. Because the distribution of $(\epsilon,\eta)$ is absolutely continuous with respect to the Lebesgue measure, $(\hat{\epsilon},\hat{\eta})\mid \cD^{(m)}_{tr}$ and $(\epsilon,\hat{\eta})\mid \cD^{(m)}_{tr}$ are also absolutely continuous\footnote{Given any training set configuration, the vectors $(\hat{\epsilon}_i,\hat{\eta}_i)$, $(\epsilon_i,\hat{\eta}_i)$, $(\hat{\epsilon}_i,\eta_i)$ are given by the sum of two independent random vectors where at least one of them is continuous because of Assumption \ref{assump:assump2_resit} and therefore the sum must be continuous, \eg, $(\hat{\epsilon}_i,\hat{\eta}_i)=(\epsilon_i,\eta_i)+(g^*_{1,P}(Z_i) -\hat{g}^{(m)}_{1}(Z_i)-\delta_{1,P}(Z_i),g^*_{2,P}(Z_i) -\hat{g}^{(m)}_{2}(Z_i)-\delta_{2,P}(Z_i))$. See Lemma \ref{lemma:lemma3_resit} for a proof.} for every training set configuration, and then we can apply Lemma \ref{lemma:lemma1_resit} to get that
\[
d_{\textup{TV}}\bigg(((\boldsymbol{\hat{\epsilon}},\boldsymbol{\hat{\eta}}),(\boldsymbol{\hat{\epsilon}},\boldsymbol{\hat{\eta}})^{(1)},\cdots,(\boldsymbol{\hat{\epsilon}},\boldsymbol{\hat{\eta}})^{(B)})\mid \cD^{(m)}_{tr},((\boldsymbol{\epsilon},\boldsymbol{\hat{\eta}}),(\boldsymbol{\epsilon},\boldsymbol{\hat{\eta}})^{(1)},\cdots,(\boldsymbol{\epsilon},\boldsymbol{\hat{\eta}})^{(B)})\mid \cD^{(m)}_{tr}\bigg)=d_{\textup{TV}}\bigg((\boldsymbol{\hat{\epsilon}},\boldsymbol{\hat{\eta}})\mid \cD^{(m)}_{tr},(\boldsymbol{\epsilon},\boldsymbol{\hat{\eta}})\mid \cD^{(m)}_{tr}\bigg).
\]
In the last step, we abuse TV distance notation: by the TV distance of two random variables, we mean the TV distance of their distributions. 

Now, define the event $$A_\alpha\triangleq\left\{((\boldsymbol{e},\boldsymbol{h}),(\boldsymbol{e},\boldsymbol{h})^{(1)},\cdots,(\boldsymbol{e},\boldsymbol{h})^{(B)}): \frac{1+\sum_{b=1}^B\ones[\Psi((\boldsymbol{e},\boldsymbol{h})^{(b)})\geq\Psi((\boldsymbol{e},\boldsymbol{h}))]}{1+B} \leq \alpha\right\}$$
By the definition of the TV distance, we have that (under $H_0$):
\begin{align*}
    \Ex_P[\varphi^{\textup{RESIT}}_\alpha(\cD^{(n)}_{te}, \cD^{(m)}_{tr})\mid \cD^{(m)}_{tr}]&=\Pr_P\left(((\boldsymbol{\hat{\epsilon}},\boldsymbol{\hat{\eta}}),(\boldsymbol{\hat{\epsilon}},\boldsymbol{\hat{\eta}})^{(1)},\cdots,(\boldsymbol{\hat{\epsilon}},\boldsymbol{\hat{\eta}})^{(B)}) \in A_\alpha \mid \cD^{(m)}_{tr}\right)\\
    &\leq \Pr_P\left(((\boldsymbol{\epsilon},\boldsymbol{\hat{\eta}}),(\boldsymbol{\epsilon},\boldsymbol{\hat{\eta}})^{(1)},\cdots,(\boldsymbol{\epsilon},\boldsymbol{\hat{\eta}})^{(B)}) \in A_\alpha \mid \cD^{(m)}_{tr}\right) + d_{\textup{TV}}\bigg((\boldsymbol{\hat{\epsilon}},\boldsymbol{\hat{\eta}})\mid \cD^{(m)}_{tr},(\boldsymbol{\epsilon},\boldsymbol{\hat{\eta}})\mid \cD^{(m)}_{tr}\bigg)\\
    &\leq\alpha + d_{\textup{TV}}\bigg((\boldsymbol{\hat{\epsilon}},\boldsymbol{\hat{\eta}})\mid \cD^{(m)}_{tr},(\boldsymbol{\epsilon},\boldsymbol{\hat{\eta}})\mid \cD^{(m)}_{tr}\bigg)\\
    &=\alpha + d_{\textup{TV}}\left(P_{\hat{\epsilon},\hat{\eta}\mid \cD^{(m)}_{tr}}^n,P_{\epsilon,\hat{\eta}\mid \cD^{(m)}_{tr}}^n\right)
\end{align*}
where the last equality holds from the fact that, given the training set, rows of $(\boldsymbol{\hat{\epsilon}},\boldsymbol{\hat{\eta}})$ and $(\boldsymbol{\epsilon},\boldsymbol{\hat{\eta}})$ are i.i.d.. See that $\Pr_P\left(((\boldsymbol{\epsilon},\boldsymbol{\hat{\eta}}),(\boldsymbol{\epsilon},\boldsymbol{\hat{\eta}})^{(1)},\cdots,(\boldsymbol{\epsilon},\boldsymbol{\hat{\eta}})^{(B)}) \in A_\alpha \mid \cD^{(m)}_{tr}\right) \leq\alpha$ because $H_0$ holds and therefore $\epsilon_i \indep \hat{\eta_i} \mid \cD^{(m)}_{tr}$ (making the permuted samples exchangeable). 

Using symmetry, we have that
\begin{align*}
    \Ex_P[\varphi^{\textup{RESIT}}_\alpha(\cD^{(n)}_{te}, \cD^{(m)}_{tr}) \mid \cD^{(m)}_{tr}]\leq \alpha + \min \left\{d_{\textup{TV}}\left(P_{\hat{\epsilon},\hat{\eta}\mid \cD^{(m)}_{tr}}^n,P_{\epsilon,\hat{\eta}\mid \cD^{(m)}_{tr}}^n\right),d_{\textup{TV}}\left(P_{\hat{\epsilon},\hat{\eta}\mid \cD^{(m)}_{tr}}^n,P_{\hat{\epsilon},\eta\mid \cD^{(m)}_{tr}}^n\right)\right\}
\end{align*}
%Because $H_0$ holds, we have that $\boldsymbol{\epsilon}\indep \boldsymbol{\eta}$ and consequently $\boldsymbol{\hat{\epsilon}}\indep \boldsymbol{\hat{\eta}}\mid \cD^{(m)}_{tr}$ and $\boldsymbol{\epsilon}\indep \boldsymbol{\hat{\eta}}\mid \cD^{(m)}_{tr}$. Then, we can applying Lemma \ref{lemma:lemma1_resit}, we get
%\begin{align*}
%    \min \left\{d_{\textup{TV}}\left(P_{\hat{\epsilon},\hat{\eta}\mid \cD^{(m)}_{tr}}^n,P_{\epsilon,\hat{\eta}\mid \cD^{(m)}_{tr}}^n\right),d_{\textup{TV}}\left(P_{\hat{\epsilon},\hat{\eta}\mid \cD^{(m)}_{tr}}^n,P_{\hat{\epsilon},\eta\mid \cD^{(m)}_{tr}}^n\right)\right\}= \min \left\{d_{\textup{TV}}\left(P_{\hat{\epsilon} \mid \cD^{(m)}_{tr}}^n,P_{\epsilon}^n\right),d_{\textup{TV}}\left(P_{\hat{\eta}\mid \cD^{(m)}_{tr}}^n,P_{\eta}^n\right)\right\}
%\end{align*}
%and the proof is complete.
\end{proof}


\end{lemma}

\begin{lemma}\label{lemma:lemma3_resit}
    For any $i\in[n]$, consider that
    \begin{align*}
        &(\hat{\epsilon}_i,\hat{\eta}_i) \mid \cD^{(m)}_{tr} \sim P_{\hat{\epsilon},\hat{\eta}\mid \cD^{(m)}_{tr}},~~ (\epsilon_i,\hat{\eta}_i) \mid \cD^{(m)}_{tr} \sim P_{\epsilon,\hat{\eta}\mid \cD^{(m)}_{tr}},~~(\hat{\epsilon}_i,\eta_i) \mid \cD^{(m)}_{tr} \sim P_{\hat{\epsilon},\eta\mid \cD^{(m)}_{tr}}
    \end{align*}
    \begin{align*}
        &(\epsilon^*_i,\eta^*_i)  \sim P_{\epsilon^*,\eta^*},~~ (\epsilon_i,\eta^*_i)  \sim P_{\epsilon,\eta^*},~~ (\epsilon^*_i,\eta_i) \sim P_{\epsilon^*,\eta}
    \end{align*}
    where $\hat{\epsilon}_i=\epsilon_i -\delta_{1,P}(Z_i) - \left(\hat{g}^{(m)}_{1}(Z_i)-g^*_{1,P}(Z_i)\right)$, $\epsilon^*_i=\epsilon_i -\delta_{1,P}(Z_i)$, $\hat{\eta}_i=\eta_i -\delta_{2,P}(Z_i) - \left(\hat{g}^{(m)}_{2}(Z_i)-g^*_{2,P}(Z_i)\right)$, and $\eta^*_i=\eta_i -\delta_{2,P}(Z_i)$. Then, under $H_0:X\indep Y\mid Z$ and Assumptions \ref{assump:assump1_resit} and \ref{assump:assump2_resit}, all six distributions are absolutely continuous with respect to the Lebesgue measure and their densities are given by
\begin{align*}
    &p_{\hat{\epsilon},\hat{\eta}\mid \cD^{(m)}_{tr}}(e,h\mid \cD^{(m)}_{tr})=\Ex_P\left[p_{\epsilon}\left(e+\delta_{1,P}(Z)+\hat{g}^{(m)}_{1}(Z)-g^*_{1,P}(Z)\right) p_{\eta}\left(h+\delta_{2,P}(Z)+\hat{g}^{(m)}_{2}(Z)-g^*_{2,P}(Z)\right)\mid \cD^{(m)}_{tr} \right]\\
    &p_{\epsilon,\hat{\eta}\mid \cD^{(m)}_{tr}}(e,h\mid \cD^{(m)}_{tr})=p_{\epsilon}(e) \cdot \Ex_P\left[p_{\eta}\left(h+\delta_{2,P}(Z)+\hat{g}^{(m)}_{2}(Z)-g^*_{2,P}(Z)\right)\mid \cD^{(m)}_{tr} \right]\\
    &p_{\hat{\epsilon},\eta\mid \cD^{(m)}_{tr}}(e,h\mid \cD^{(m)}_{tr})=\Ex_P\left[p_{\epsilon}\left(e+\delta_{1,P}(Z)+\hat{g}^{(m)}_{1}(Z)-g^*_{1,P}(Z)\right) \mid \cD^{(m)}_{tr} \right]\cdot p_{\eta}(h)\\
    &p_{\epsilon^*,\eta^*}(e,h)=\Ex_P\left[p_{\epsilon}\left(e+\delta_{1,P}(Z)\right) p_{\eta}\left(h+\delta_{2,P}(Z)\right) \right]\\
    &p_{\epsilon,\eta^*}(e,h)=p_{\epsilon}(e) \cdot \Ex_P\left[p_{\eta}\left(h+\delta_{2,P}(Z)\right) \right]\\
    &p_{\epsilon^*,\eta}(e,h)=\Ex_P\left[p_{\epsilon}\left(e+\delta_{1,P}(Z)\right) \right]\cdot p_{\eta}(h)
\end{align*}

Additionally, we have that
 \begin{align*}
    &\sup_{(e,h)\in \reals^{d_X \times d_Y}} \left(p_{\hat{\epsilon},\hat{\eta}\mid \cD^{(m)}_{tr}}(e,h\mid \cD^{(m)}_{tr})-p_{\epsilon^*,\eta^*}(e,h)\right)^2=\cO_{\cP_0}(m^{-\gamma})\\
    &\sup_{(e,h)\in \reals^{d_X \times d_Y}} \left(p_{\epsilon,\hat{\eta}\mid \cD^{(m)}_{tr}}(e,h\mid \cD^{(m)}_{tr})-p_{\epsilon,\eta^*}(e,h)\right)^2=\cO_{\cP_0}(m^{-\gamma})\\
    &\sup_{(e,h)\in \reals^{d_X \times d_Y}} \left(p_{\hat{\epsilon},\eta\mid \cD^{(m)}_{tr}}(e,h\mid \cD^{(m)}_{tr})-p_{\epsilon^*,\eta}(e,h)\right)^2=\cO_{\cP_0}(m^{-\gamma})
\end{align*}
\begin{proof}
    
Assume we are under $H_0$. In order to show that $P_{\hat{\epsilon},\hat{\eta}\mid \cD^{(m)}_{tr}}$ is absolutely continuous w.r.t. Lebesgue measure (for each training set configuration) and that its density is given by 
\[
p_{\hat{\epsilon},\hat{\eta}\mid \cD^{(m)}_{tr}}(e,h\mid \cD^{(m)}_{tr})=\Ex_P\left[p_{\epsilon}\left(e+\delta_{1,P}(Z)+\hat{g}^{(m)}_{1}(Z)-g^*_{1,P}(Z)\right) p_{\eta}\left(h+\delta_{2,P}(Z)+\hat{g}^{(m)}_{2}(Z)-g^*_{2,P}(Z)\right)\mid \cD^{(m)}_{tr} \right],
\]
it suffices to show that 
\begin{align*}
 &\Pr_P((\hat{\epsilon},\hat{\eta})\in A \mid \cD^{(m)}_{tr})=\\
 &=\int \ones_A(u,v) \Ex_P\left[p_{\epsilon}\left(u+\delta_{1,P}(Z)+\hat{g}^{(m)}_{1}(Z)-g^*_{1,P}(Z)\right) p_{\eta}\left(v+\delta_{2,P}(Z)+\hat{g}^{(m)}_{2}(Z)-g^*_{2,P}(Z)\right)\mid \cD^{(m)}_{tr} \right]d(u,v)   
\end{align*}
for any measurable set $A$. 

Using Fubini's theorem, we get
\begin{align*}
    &\Pr_P((\hat{\epsilon},\hat{\eta})\in A \mid \cD^{(m)}_{tr})=\\
    &= \Ex_P\left[\ones_A(\epsilon-\delta_{1,P}(Z)-\hat{g}^{(m)}_{1}(Z)+g^*_{1,P}(Z),\eta-\delta_{2,P}(Z)-\hat{g}^{(m)}_{2}(Z)+g^*_{2,P}(Z)) \mid \cD^{(m)}_{tr}  \right]\\
    &= \Ex_P\left[\int \ones_A(e-\delta_{1,P}(Z)-\hat{g}^{(m)}_{1}(Z)+g^*_{1,P}(Z),h-\delta_{2,P}(Z)-\hat{g}^{(m)}_{2}(Z)+g^*_{2,P}(Z))p_{\epsilon,\eta}(e,h) d(e,h) \mid \cD^{(m)}_{tr}  \right]\\
    &= \Ex_P\left[\int \ones_A(e-\delta_{1,P}(Z)-\hat{g}^{(m)}_{1}(Z)+g^*_{1,P}(Z),h-\delta_{2,P}(Z)-\hat{g}^{(m)}_{2}(Z)+g^*_{2,P}(Z))p_{\epsilon}(e)p_{\eta}(h) d(e,h) \mid \cD^{(m)}_{tr}  \right]\\
    &= \Ex_P\left[\int \ones_A(u,v)p_{\epsilon}\left(u+\delta_{1,P}(Z)+\hat{g}^{(m)}_{1}(Z)-g^*_{1,P}(Z)\right)p_{\eta}\left(v+\delta_{2,P}(Z)+\hat{g}^{(m)}_{2}(Z)-g^*_{2,P}(Z)\right) d(u,v) \mid \cD^{(m)}_{tr}  \right]\\
    &= \int \ones_A(u,v) \Ex_P\left[p_{\epsilon}\left(u+\delta_{1,P}(Z)+\hat{g}^{(m)}_{1}(Z)-g^*_{1,P}(Z)\right) p_{\eta}\left(v+\delta_{2,P}(Z)+\hat{g}^{(m)}_{2}(Z)-g^*_{2,P}(Z)\right)\mid \cD^{(m)}_{tr} \right]d(u,v)   
\end{align*}

The proof is analogous to the other distributions. 

Now, we proceed with the second part of the lemma. Using Assumptions \ref{assump:assump1_resit} and \ref{assump:assump2_resit}, we get
\begin{align*}
    &\left(p_{\hat{\epsilon},\hat{\eta}\mid \cD^{(m)}_{tr}}(e,h\mid \cD^{(m)}_{tr})-p_{\epsilon^*,\eta^*}(e,h)\right)^2=\\
    &=\Big(\Ex_P\Big[p_{\epsilon}\left(e+\delta_{1,P}(Z)+\hat{g}^{(m)}_{1}(Z)-g^*_{1,P}(Z)\right) p_{\eta}\left(h+\delta_{2,P}(Z)+\hat{g}^{(m)}_{2}(Z)-g^*_{2,P}(Z)\right)\\
    &~~~~~~~~~~~~~ -p_{\epsilon}\left(e+\delta_{1,P}(Z)\right) p_{\eta}\left(h+\delta_{2,P}(Z)\right) \mid \cD^{(m)}_{tr} \Big]\Big)^2\\
    &\leq L^2 \left(\Ex_P\left[\norm{\left(\hat{g}^{(m)}_{1}(Z)-g^*_{1}(Z),\hat{g}^{(m)}_{2}(Z)-g^*_{2}(Z)\right)}_2 \mid \cD^{(m)}_{tr}\right]\right)^2\\
    &\leq L^2 \left(\Ex_P\left[\norm{\left(\hat{g}^{(m)}_{1}(Z)-g^*_{1}(Z),\hat{g}^{(m)}_{2}(Z)-g^*_{2}(Z)\right)}^2_2 \mid \cD^{(m)}_{tr}\right]\right)\\
    &= L^2 \Ex_P\left[\norm{\hat{g}^{(m)}_{1}(Z)-g^*_{1,P}(Z)}_2^2 \mid \cD^{(m)}_{tr}\right]+L^2 \Ex_P\left[\norm{\hat{g}^{(m)}_{2}(Z)-g^*_{2,P}(Z)}_2^2 \mid \cD^{(m)}_{tr}\right]\\
    &=\cO_{\cP_0}(m^{-\gamma})
\end{align*}
where the last inequality is obtained via Jensen's inequality. Because the convergence rate does not depend on $(e,h)$, we get
 \begin{align*}
    \sup_{(e,h)\in \reals^{d_X \times d_Y}} \left(p_{\hat{\epsilon},\hat{\eta}\mid \cD^{(m)}_{tr}}(e,h\mid \cD^{(m)}_{tr})-p_{\epsilon^*,\eta^*}(e,h)\right)^2=\cO_{\cP_0}(m^{-\gamma})
\end{align*}
The results for the other converging quantities are obtained in the same manner.
\end{proof}
\end{lemma}


\textbf{Theorem \ref{thm:thm1_resit}.} Under Assumptions \ref{assump:assump1_resit}, \ref{assump:assump2_resit}, and \ref{assump:assump3_resit}, if $H_0:X\indep Y\mid Z$ holds and $n$ is a function of $m$ such that $n\to \infty$ and $n=o(m^\frac{\gamma}{2})$ as $m\to \infty$,  then
    \begin{align*}
    \Ex_P[\varphi^{\textup{RESIT}}_\alpha(\cD^{(n)}_{te}, \cD^{(m)}_{tr})]\leq \alpha + \min\{d_\text{TV}(P^n_{\epsilon^*,\eta^*},P^n_{\epsilon,\eta^*}), d_\text{TV}(P^n_{\epsilon^*,\eta^*},P^n_{\epsilon^*,\eta})\} +o(1)
    \end{align*}
    where $o(1)$ denotes uniform convergence over all $P \in \cP_0$ as $m\to \infty$.
    
\begin{proof}

We are trying to prove that
\[
\sup_{P\in\cP_0}\left[\Ex_P[\varphi^{\textup{RESIT}}_\alpha(\cD^{(n)}_{te}, \cD^{(m)}_{tr})]-\alpha- \min\{d_\text{TV}(P^n_{\epsilon^*,\eta^*},P^n_{\epsilon,\eta^*}), d_\text{TV}(P^n_{\epsilon^*,\eta^*},P^n_{\epsilon^*,\eta})\}\right]\leq o(1)\text{ as $m\to\infty$}
\]

First, see that using Lemma \ref{lemma:lemma2_resit} we get
\begin{align*}
    &\Ex_P[\varphi^{\textup{RESIT}}_\alpha(\cD^{(n)}_{te}, \cD^{(m)}_{tr})]=\\
    &=\Ex_P[\Ex_P[\varphi^{\textup{RESIT}}_\alpha(\cD^{(n)}_{te}, \cD^{(m)}_{tr}) \mid \cD^{(m)}_{tr}]]\\
    &\leq \alpha + \Ex_P\left[\min \left\{d_{\textup{TV}}\left(P_{\hat{\epsilon}, \hat{\eta} \mid \cD^{(m)}_{tr}}^n,P_{\epsilon, \hat{\eta} \mid \cD^{(m)}_{tr}}^n\right),d_{\textup{TV}}\left(P_{\hat{\epsilon}, \hat{\eta} \mid \cD^{(m)}_{tr}}^n,P_{\hat{\epsilon}, \eta \mid \cD^{(m)}_{tr}}^n\right)\right\}\right]\\
    &\leq \alpha + \min \left\{\Ex_P\left[d_{\textup{TV}}\left(P_{\hat{\epsilon}, \hat{\eta} \mid \cD^{(m)}_{tr}}^n,P_{\epsilon, \hat{\eta} \mid \cD^{(m)}_{tr}}^n\right)\right],\Ex_P\left[d_{\textup{TV}}\left(P_{\hat{\epsilon}, \hat{\eta} \mid \cD^{(m)}_{tr}}^n,P_{\hat{\epsilon}, \eta \mid \cD^{(m)}_{tr}}^n\right)\right]\right\}\\
    &\leq \alpha + \min \Bigg\{\Ex_P\left[d_{\textup{TV}}\left(P_{\hat{\epsilon}, \hat{\eta} \mid \cD^{(m)}_{tr}}^n,P_{\epsilon, \hat{\eta} \mid \cD^{(m)}_{tr}}^n\right)\right]-d_\text{TV}(P^n_{\epsilon^*,\eta^*},P^n_{\epsilon,\eta^*})+d_\text{TV}(P^n_{\epsilon^*,\eta^*},P^n_{\epsilon,\eta^*}),\\
    &~~~~~~~~~~~~~~~~~~~~~~ \Ex_P\left[d_{\textup{TV}}\left(P_{\hat{\epsilon}, \hat{\eta} \mid \cD^{(m)}_{tr}}^n,P_{\hat{\epsilon}, \eta \mid \cD^{(m)}_{tr}}^n\right)-d_\text{TV}(P^n_{\epsilon^*,\eta^*},P^n_{\epsilon^*,\eta})+d_\text{TV}(P^n_{\epsilon^*,\eta^*},P^n_{\epsilon^*,\eta})\right]\Bigg\}\\
    &\leq \alpha + \min \Bigg\{\left|\Ex_P\left[d_{\textup{TV}}\left(P_{\hat{\epsilon}, \hat{\eta} \mid \cD^{(m)}_{tr}}^n,P_{\epsilon, \hat{\eta} \mid \cD^{(m)}_{tr}}^n\right)\right]-d_\text{TV}(P^n_{\epsilon^*,\eta^*},P^n_{\epsilon,\eta^*})\right|+d_\text{TV}(P^n_{\epsilon^*,\eta^*},P^n_{\epsilon,\eta^*}),\\
    &~~~~~~~~~~~~~~~~~~~~~~ \left|\Ex_P\left[d_{\textup{TV}}\left(P_{\hat{\epsilon}, \hat{\eta} \mid \cD^{(m)}_{tr}}^n,P_{\hat{\epsilon}, \eta \mid \cD^{(m)}_{tr}}^n\right)-d_\text{TV}(P^n_{\epsilon^*,\eta^*},P^n_{\epsilon^*,\eta})\right|+d_\text{TV}(P^n_{\epsilon^*,\eta^*},P^n_{\epsilon^*,\eta})\right]\Bigg\}
\end{align*}
and
\begin{align}
 &\sup_{P\in\cP_0}\left[\Ex_P[\varphi^{\textup{RESIT}}_\alpha(\cD^{(n)}_{te}, \cD^{(m)}_{tr})]-\alpha- \min\{d_\text{TV}(P^n_{\epsilon^*,\eta^*},P^n_{\epsilon,\eta^*}), d_\text{TV}(P^n_{\epsilon^*,\eta^*},P^n_{\epsilon^*,\eta})\}\right]\leq \sup_{P\in\cP_0}\Delta_P^{(m)}\label{step:step1_resit}
\end{align}
where
\begin{align*}
\Delta_P^{(m)}&\triangleq \min \Bigg\{\left|\Ex_P\left[d_{\textup{TV}}\left(P_{\hat{\epsilon}, \hat{\eta} \mid \cD^{(m)}_{tr}}^n,P_{\epsilon, \hat{\eta} \mid \cD^{(m)}_{tr}}^n\right)\right]-d_\text{TV}(P^n_{\epsilon^*,\eta^*},P^n_{\epsilon,\eta^*})\right|+d_\text{TV}(P^n_{\epsilon^*,\eta^*},P^n_{\epsilon,\eta^*}),\\
&~~~~~~~~~~~~~~~ \left|\Ex_P\left[d_{\textup{TV}}\left(P_{\hat{\epsilon}, \hat{\eta} \mid \cD^{(m)}_{tr}}^n,P_{\hat{\epsilon}, \eta \mid \cD^{(m)}_{tr}}^n\right)\right]-d_\text{TV}(P^n_{\epsilon^*,\eta^*},P^n_{\epsilon^*,\eta})\right|+d_\text{TV}(P^n_{\epsilon^*,\eta^*},P^n_{\epsilon^*,\eta})\Bigg\}\\
&~~~~~~~~~~~~~~~ - \min\{d_\text{TV}(P^n_{\epsilon^*,\eta^*},P^n_{\epsilon,\eta^*}), d_\text{TV}(P^n_{\epsilon^*,\eta^*},P^n_{\epsilon^*,\eta})\} 
\end{align*}


It suffices to show that $\sup_{P\in\cP_0}\Delta_P^{(m)}=o(1)$ as $m\to\infty$. Next step is to show that
\[
\sup_{P\in\cP_0}\left|\Ex_P\left[d_{\textup{TV}}\left(P_{\hat{\epsilon}, \hat{\eta} \mid \cD^{(m)}_{tr}}^n,P_{\epsilon, \hat{\eta} \mid \cD^{(m)}_{tr}}^n\right)\right] - d_\text{TV}(P^n_{\epsilon^*,\eta^*},P^n_{\epsilon,\eta^*})\right|=o(1)
\]
and
\[
\sup_{P\in\cP_0}\left|\Ex_P\left[d_{\textup{TV}}\left(P_{\hat{\epsilon}, \hat{\eta} \mid \cD^{(m)}_{tr}}^n,P_{\hat{\epsilon}, \eta \mid \cD^{(m)}_{tr}}^n\right)\right] - d_\text{TV}(P^n_{\epsilon^*,\eta^*},P^n_{\epsilon^*,\eta})\right|=o(1)
\]
as $m\to \infty$. Given the symmetry, we focus on the first problem.

By the triangle inequality, we obtain
\[
 \Ex_P\left[d_{\textup{TV}}\left(P_{\hat{\epsilon},\hat{\eta} \mid \cD^{(m)}_{tr}}^n,P_{\epsilon,\hat{\eta}\mid \cD^{(m)}_{tr}}^n\right)\right] \leq \Ex_P\left[d_{\textup{TV}}\left(P_{\hat{\epsilon},\hat{\eta} \mid \cD^{(m)}_{tr}}^n,P_{\epsilon^*,\eta^*}^n\right)\right]+ d_{\textup{TV}}\left(P_{\epsilon^*,\eta^* }^n,P_{\epsilon,\eta^*}^n\right)+ \Ex_P\left[d_{\textup{TV}}\left(P_{\epsilon,\eta^*}^n,P_{\epsilon,\hat{\eta}\mid \cD^{(m)}_{tr}}^n\right)\right]
\]
and consequently
\begin{align*}
  &\sup_{P\in\cP_0}\left|\Ex_P\left[d_{\textup{TV}}\left(P_{\hat{\epsilon},\hat{\eta} \mid \cD^{(m)}_{tr}}^n,P_{\epsilon,\hat{\eta}\mid \cD^{(m)}_{tr}}^n\right)\right] - d_{\textup{TV}}\left(P_{\epsilon^*,\eta^* }^n,P_{\epsilon,\eta^*}^n\right)\right| \\
  &\leq \underbrace{\sup_{P\in\cP_0}\Ex_P\left[d_{\textup{TV}}\left(P_{\hat{\epsilon},\hat{\eta} \mid \cD^{(m)}_{tr}}^n,P_{\epsilon^*,\eta^*}^n\right)\right]}_{\text{I}}  +\underbrace{\sup_{P\in\cP_0}\Ex_P\left[d_{\textup{TV}}\left(P_{\epsilon,\hat{\eta}\mid \cD^{(m)}_{tr}}^n,P_{\epsilon,\eta^*}^n\right)\right]}_{\text{II}}  
\end{align*}
We treat these terms separately.

(I) Consider a sequence of probability distributions $(P^{(m)})_{m\in\mathbb{N}}$ in $\cP_0$ such that
\[
\sup_{P \in \cP_0} \Ex_P\left[d_{\textup{TV}}\left(P_{\hat{\epsilon},\hat{\eta} \mid \cD^{(m)}_{tr}}^n,P_{\epsilon^*,\eta^*}^n\right)\right]\leq \Ex_{P^{(m)}}\left[d_{\textup{TV}}\left({P^{(m)}}_{\hat{\epsilon},\hat{\eta} \mid \cD^{(m)}_{tr}}^n,{P^{(m)}}_{\epsilon^*,\eta^*}^n\right)\right] + \frac{1}{m}
\]
Here, the distributions $P$ and $P^{(m)}$ determine not only the distribution associated with $\cD^{(m)}_{tr}$ but also the distribution of $(\hat{\epsilon},\hat{\eta},\epsilon^*,\eta^*)$. Because we have that
\begin{align*}
   &d_{\textup{TV}}\left(P_{\hat{\epsilon},\hat{\eta} \mid \cD^{(m)}_{tr}}^n,P_{\epsilon^*,\eta^*}^n\right)\leq\\
   &\leq n\cdot  d_{\textup{TV}}\left(P_{\hat{\epsilon},\hat{\eta} \mid \cD^{(m)}_{tr}},P_{\epsilon^*,\eta^*}\right) ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ (\text{Subadditivity of TV distance}) \\
        &= \frac{n}{2}\int \left|p_{\hat{\epsilon},\hat{\eta} \mid \cD^{(m)}_{tr}}(e,h\mid \cD^{(m)}_{tr}) -p_{\epsilon^*,\eta^*}(e,h) \right|  d(u,v) ~~~~~~~~~~~ (\text{Scheffe's theorem \citep{tsybakov2004introduction2}[Lemma 2.1]})\\
        &\leq \frac{n V}{2} \sup_{(u,v)\in \reals^{d_X\times d_Y}} \left|p_{\hat{\epsilon},\hat{\eta} \mid \cD^{(m)}_{tr}}(e,h\mid \cD^{(m)}_{tr}) -p_{\epsilon^*,\eta^*}(e,h) \right| ~~ (\text{Assumption \ref{assump:assump3_resit}})\\
        &= \left(n^2V^2 \sup_{(u,v)\in \reals^{d_X\times d_Y}} \left|p_{\hat{\epsilon},\hat{\eta} \mid \cD^{(m)}_{tr}}(e,h\mid \cD^{(m)}_{tr}) -p_{\epsilon^*,\eta^*}(e,h) \right|^2\right)^{1/2} \\
        &= \left(o(m^{\gamma}) \cO_{\cP_0}(m^{-\gamma})\right)^{1/2} ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ (\text{Lemma \ref{lemma:lemma3_resit}})\\
        &=o_{\cP_0}(1)
\end{align*}
where $V$ is the volume of a ball containing the support of the RVs (existence of that ball is due to \text{Assumption \ref{assump:assump3_resit}}). We also have that $d_{\textup{TV}}\left({P^{(m)}}_{\hat{\epsilon},\hat{\eta} \mid \cD^{(m)}_{tr}}^n,{P^{(m)}}_{\epsilon^*,\eta^*}^n\right)=o_p(1)$, when $\cD^{(m)}_{tr}$ samples come from the sequence$(P^{(m)})_{m\in\mathbb{N}}$. By the Dominated Convergence Theorem (DCT) \citep[Corollary 6.3.2]{resnick2019probability}, we have
\[
\sup_{P \in \cP_0} \Ex_P\left[d_{\textup{TV}}\left(P_{\hat{\epsilon},\hat{\eta} \mid \cD^{(m)}_{tr}}^n,P_{\epsilon^*,\eta^*}^n\right)\right]\leq \Ex_{P^{(m)}}\left[d_{\textup{TV}}\left({P^{(m)}}_{\hat{\epsilon},\hat{\eta} \mid \cD^{(m)}_{tr}}^n,{P^{(m)}}_{\epsilon^*,\eta^*}^n\right)\right] + \frac{1}{m}=o(1)
\]

To see why we can use the DCT here, realize that when samples come from $P^{(m)}$, $W^{(m)}=d_{\textup{TV}}\left({P^{(m)}}_{\hat{\epsilon},\hat{\eta} \mid \cD^{(m)}_{tr}}^n,{P^{(m)}}_{\epsilon^*,\eta^*}^n\right)$ can be seen as a measurable function going from an original probability space to some other space. Different distributions $\{P^{(m)}\}$ are due to different random variables while the original probability measure is fixed. Because of that,
\[
\Ex_{P^{(m)}}\left[d_{\textup{TV}}\left({P^{(m)}}_{\hat{\epsilon},\hat{\eta} \mid \cD^{(m)}_{tr}}^n,{P^{(m)}}_{\epsilon^*,\eta^*}^n\right)\right] = \Ex\left[W^{(m)}\right] 
\]
for the bounded random variable $W^{(m)}$, where the last expectation is taken in the original probability space.

(II) Following the same steps as in part (I), we obtain
\[
\sup_{P \in \cP_0} \Ex_P\left[d_{\textup{TV}}\left(P_{\epsilon,\hat{\eta} \mid \cD^{(m)}_{tr}}^n,P_{\epsilon,\eta^*}^n\right)\right]=o(1)
\]
Going back to step \ref{step:step1_resit}, consider another sequence of probability distributions $(Q^{(m)})_{m\in\mathbb{N}}$ in $\cP_0$ such that
\[
\sup_{P\in\cP_0}\Delta_P^{(m)}\leq \Delta_{Q^{(m)}}^{(m)} + \frac{1}{m}
\]
where
\begin{align*}
\Delta_{Q^{(m)}}^{(m)}=& \min \Bigg\{\left|\Ex_{Q^{(m)}}\left[d_{\textup{TV}}\left({Q^{(m)}}_{\hat{\epsilon}, \hat{\eta} \mid \cD^{(m)}_{tr}}^n,{Q^{(m)}}_{\epsilon, \hat{\eta} \mid \cD^{(m)}_{tr}}^n\right)\right]-d_\text{TV}({Q^{(m)}}^n_{\epsilon^*,\eta^*},{Q^{(m)}}^n_{\epsilon,\eta^*})\right|+d_\text{TV}({Q^{(m)}}^n_{\epsilon^*,\eta^*},{Q^{(m)}}^n_{\epsilon,\eta^*}),\\
&~~~~~~~~~~~ \left|\Ex_{Q^{(m)}}\left[d_{\textup{TV}}\left({Q^{(m)}}_{\hat{\epsilon}, \hat{\eta} \mid \cD^{(m)}_{tr}}^n,{Q^{(m)}}_{\hat{\epsilon}, \eta \mid \cD^{(m)}_{tr}}^n\right)-d_\text{TV}({Q^{(m)}}^n_{\epsilon^*,\eta^*},{Q^{(m)}}^n_{\epsilon^*,\eta})\right|+d_\text{TV}({Q^{(m)}}^n_{\epsilon^*,\eta^*},{Q^{(m)}}^n_{\epsilon^*,\eta})\right]\Bigg\}\\
&~~~~ - \min\{d_\text{TV}({Q^{(m)}}^n_{\epsilon^*,\eta^*},{Q^{(m)}}^n_{\epsilon,\eta^*}), d_\text{TV}({Q^{(m)}}^n_{\epsilon^*,\eta^*},{Q^{(m)}}^n_{\epsilon^*,\eta})\} 
\end{align*}

Because of continuity of $\min$ and
\[
\sup_{P\in\cP_0}\left|\Ex_P\left[d_{\textup{TV}}\left(P_{\hat{\epsilon}, \hat{\eta} \mid \cD^{(m)}_{tr}}^n,P_{\epsilon, \hat{\eta} \mid \cD^{(m)}_{tr}}^n\right)\right] - d_\text{TV}(P^n_{\epsilon^*,\eta^*},P^n_{\epsilon,\eta^*})\right|=o(1)
\]
and
\[
\sup_{P\in\cP_0}\left|\Ex_P\left[d_{\textup{TV}}\left(P_{\hat{\epsilon}, \hat{\eta} \mid \cD^{(m)}_{tr}}^n,P_{\hat{\epsilon}, \eta \mid \cD^{(m)}_{tr}}^n\right)\right] - d_\text{TV}(P^n_{\epsilon^*,\eta^*},P^n_{\epsilon^*,\eta})\right|=o(1)
\]
we have that
\begin{align*}
&\Delta_{Q^{(m)}}^{(m)}=\\
&=\min\{d_\text{TV}({Q^{(m)}}^n_{\epsilon^*,\eta^*},{Q^{(m)}}^n_{\epsilon,\eta^*})+o(1), d_\text{TV}({Q^{(m)}}^n_{\epsilon^*,\eta^*},{Q^{(m)}}^n_{\epsilon^*,\eta})+o(1)\}\\
& ~~~~~ - \min\{d_\text{TV}({Q^{(m)}}^n_{\epsilon^*,\eta^*},{Q^{(m)}}^n_{\epsilon,\eta^*}), d_\text{TV}({Q^{(m)}}^n_{\epsilon^*,\eta^*},{Q^{(m)}}^n_{\epsilon^*,\eta})\}\\
&= \min\{d_\text{TV}({Q^{(m)}}^n_{\epsilon^*,\eta^*},{Q^{(m)}}^n_{\epsilon,\eta^*}), d_\text{TV}({Q^{(m)}}^n_{\epsilon^*,\eta^*},{Q^{(m)}}^n_{\epsilon^*,\eta}))\}\\
& ~~~~~ - \min\{d_\text{TV}({Q^{(m)}}^n_{\epsilon^*,\eta^*},{Q^{(m)}}^n_{\epsilon,\eta^*}), d_\text{TV}({Q^{(m)}}^n_{\epsilon^*,\eta^*},{Q^{(m)}}^n_{\epsilon^*,\eta})\}+o(1)\\
&=o(1)
\end{align*}

Finally implying, from step \ref{step:step1_resit},
 \[
\sup_{P\in\cP_0}\left[\Ex_P[\varphi^{\textup{RESIT}}_\alpha(\cD^{(n)}_{te}, \cD^{(m)}_{tr})]-\alpha- \min\{d_\text{TV}(P^n_{\epsilon^*,\eta^*},P^n_{\epsilon,\eta^*}), d_\text{TV}(P^n_{\epsilon^*,\eta^*},P^n_{\epsilon^*,\eta})\}\right]\leq o(1)\text{ as $m\to\infty$}
\]
\end{proof}

%\newgeometry{left=3cm}
\subsection{RBPT }

\textbf{Theorem \ref{thm:thm1_rbpt}.} Suppose that Assumptions \ref{assump:assump1_rbpt}, \ref{assump:assump2_rbpt}, \ref{assump:assump3_rbpt}, \ref{assump:assump2_stfr}, and \ref{assump:assump3_stfr} hold. If $n$ is a function of $m$ such that $n\to \infty$ and $n=o(m^{\gamma})$ as $m\to \infty$,  then
\begin{align*}
\Ex_P[\varphi^{\textup{RBPT}}_\alpha(\cD^{(n)}_{te},\cD_{tr}^{(m)})]=1-\Phi\left(\tau_{\alpha}-\sqrt{\frac{n}{\sigma_P^2}}\Omega_P^{\textup{RBPT}}\right) +o(1)
\end{align*}
where $o(1)$ denotes uniform convergence over all $P \in \cP$ as $m\to \infty$ and
\begin{align*}
\Omega_P^{\textup{RBPT}}=\Omega_{P,1}^{\textup{RBPT}}-\Omega_{P,2}^{\textup{RBPT}}
\end{align*}
with
\begin{align*}
   \Omega_{P,1}^{\textup{RBPT}}\triangleq \Ex_{P}&\Bigg[\ell\left(\int  g_{P}^{*}(x,Z) dQ^*_{X|Z}(x),Y\right)- \ell\left(\int  g_{P}^{*}(x,Z) dP_{X\mid Z}(x),Y\right) \Bigg]
\end{align*}
and
\begin{align*}
   \underbrace{\Omega_{P,2}^{\textup{RBPT}}}_{\text{Jensen's gap}}\triangleq \Ex_{P}&\Bigg[\ell(g_{P}^*(X,Z),Y)- \ell\left(\int g_{P}^*(x,Z) dP_{X\mid Z}(x),Y\right) \Bigg]
\end{align*}

\begin{proof}
First, note that there must be\footnote{Because of the definition of $\sup$.} a sequence of probability measures in $\cP$, $(P^{(m)})_{m\in\mathbb{N}}$, such that
\begin{align*}
   &\sup_{P\in \cP}\left|\Ex_P[\varphi^{\textup{RBPT}}_\alpha(\cD^{(n)}_{te},\cD_{tr}^{(m)})]-1+\Phi\left(\tau_{\alpha}-\sqrt{\frac{n}{\sigma_P^2}}\Omega_P^{\textup{RBPT}}\right)\right|\leq \left|\Ex_{P^{(m)}}[\varphi^{\textup{RBPT}}_\alpha(\cD^{(n)}_{te},\cD_{tr}^{(m)})]-1+\Phi\left(\tau_{\alpha}-\sqrt{\frac{n}{\sigma_{P^{(m)}}^2}}\Omega_{P^{(m)}}^{\textup{RBPT}}\right)\right| + \frac{1}{m}
\end{align*}

Then, it suffices to show that the RHS vanishes when we consider such a sequence $(P^{(m)})_{m\in\mathbb{N}}$.

Now, let us first decompose the test statistic $\Xi^{(n,m)}$ in the following way:
\begin{align*}
&\Xi^{(n,m)}\triangleq\frac{\sqrt{n}\bar{T}^{(n,m)}}{\hat{\sigma}^{(n,m)}}=\\
&=\frac{\sqrt{n}\Big(\bar{T}^{(n,m)}-\Ex_{P^{(m)}}[T^{(m)}_1 \mid \cD_{tr}^{(m)}]\Big)}{\hat{\sigma}^{(n,m)}}+\frac{\sqrt{n}\Ex_{P^{(m)}}[T^{(m)}_1 \mid \cD_{tr}^{(m)}]}{\hat{\sigma}^{(n,m)}}\\
&=\frac{\sqrt{n}\Big(\bar{T}^{(n,m)}-\Ex_{P^{(m)}}[T^{(m)}_1 \mid \cD_{tr}^{(m)}]\Big)}{\hat{\sigma}^{(n,m)}}+\frac{\sqrt{n}\Ex_{P^{(m)}}[\ell(\hat{h}(Z_1),Y_1)- \ell(\hat{g}^{(m)}(X_1,Z_1),Y_1) \mid \cD_{tr}^{(m)}]}{\hat{\sigma}^{(n,m)}}\\
&=\frac{\sqrt{n}\Big(\bar{T}^{(n,m)}-\Ex_{P^{(m)}}[T^{(m)}_1 \mid \cD_{tr}^{(m)}]\Big)}{\hat{\sigma}^{(n,m)}}+\frac{\sqrt{n}\Ex_{P^{(m)}}[\ell(\int \hat{g}^{(m)}(x,Z_1) d\hat{Q}^{(m)}_{X\mid Z}(x),Y_1)- \ell(\hat{g}^{(m)}(X_1,Z_1),Y_1) \mid \cD_{tr}^{(m)}]}{\hat{\sigma}^{(n,m)}}\\
    &=\frac{\sqrt{n}\Big(\bar{T}^{(n,m)}-\Ex_{P^{(m)}}[T^{(m)}_1 \mid \cD_{tr}^{(m)}]\Big)}{\hat{\sigma}^{(n,m)}}+\\
     &+\frac{\sqrt{n}\Ex_{P^{(m)}}[\ell(\int \hat{g}^{(m)}(x,Z_1) d\hat{Q}^{(m)}_{X\mid Z}(x),Y_1)- \ell(\int \hat{g}^{(m)}(x,Z_1) dQ^*_{X|Z}(x),Y_1) \mid \cD_{tr}^{(m)}]}{\hat{\sigma}^{(n,m)}}\\
    &+\frac{\sqrt{n}\Ex_{P^{(m)}}[\ell(\int \hat{g}^{(m)}(x,Z_1) dQ^*_{X|Z}(x),Y_1)- \ell(\int g_{P^{(m)}}^{*}(x,Z_1) dQ^*_{X|Z}(x),Y_1) \mid \cD_{tr}^{(m)}]}{\hat{\sigma}^{(n,m)}}\\
    &+\frac{\sqrt{n}\Ex_{P^{(m)}}[\ell(g_{P^{(m)}}^*(X_1,Z_1),Y_1)- \ell(\hat{g}^{(m)}(X_1,Z_1),Y_1) \mid \cD_{tr}^{(m)}]}{\hat{\sigma}^{(n,m)}}\\
    &+\frac{\sqrt{n}}{\hat{\sigma}^{(n,m)}}\Ex_{P^{(m)}}\Bigg[\Big[\ell\Big(\int  g_{P^{(m)}}^{*}(x,Z_1) dQ^*_{X|Z}(x),Y\Big)- \ell\Big(\int  g_{P^{(m)}}^{*}(x,Z_1) dP^{(m)}_{X\mid Z}(x),Y\Big)\Big] + \\
    &~~~~~~~~~~~~~~~~~~~~~~~~~~ +\Big[\ell\Big(\int g_{P^{(m)}}^*(x,Z_1) dP^{(m)}_{X\mid Z}(x),Y\Big)- \ell(g_{P^{(m)}}^*(X_1,Z_1),Y_1)\Big] \Bigg]\\
    &=\frac{\sqrt{n}W^{(m)}_{1, P^{(m)}}}{\hat{\sigma}^{(n,m)}}+\frac{\sqrt{n}W^{(m)}_{2, P^{(m)}}}{\hat{\sigma}^{(n,m)}}+\frac{\sqrt{n}W^{(m)}_{3, P^{(m)}}}{\hat{\sigma}^{(n,m)}}+\frac{\sqrt{n}W^{(m)}_{4, P^{(m)}}}{\hat{\sigma}^{(n,m)}}+\frac{\sqrt{n} \Omega_{P^{(m)}}^{\textup{RBPT}}}{\hat{\sigma}^{(n,m)}}
\end{align*}


Given that $n$ is a function of $m$, we omit it when writing the $W^{(m)}_{j,P^{(m)}}$'s. Define $\sigma_{P^{(m)}}^{(m)}\triangleq \sqrt{\Var_{P^{(m)}}[T^{(m)}_1\mid  \cD_{tr}^{(m)}]}$ and see that
\begin{align}
    &\Ex_{P^{(m)}}[\varphi^{\textup{RBPT}}_\alpha(\cD^{(n)}_{te},\cD_{tr}^{(m)}) ]=\\
    &=\Pr_{P^{(m)}}[p(\cD^{(n)}_{te},\cD_{tr}^{(m)})\leq \alpha] \nonumber\\
    &=\Pr_{P^{(m)}}\left[1-\Phi\left(\Xi^{(n,m)}\right)\leq \alpha \right] \nonumber\\
    &=\Pr_{P^{(m)}}\left[\Xi^{(n,m)} \geq \tau_\alpha \right] \nonumber\\
    &=\Pr_{P^{(m)}}\left[\frac{\sqrt{n}W^{(m)}_{1, P^{(m)}}}{\hat{\sigma}^{(n,m)}}+\frac{\sqrt{n}W^{(m)}_{2, P^{(m)}}}{\hat{\sigma}^{(n,m)}}+\frac{\sqrt{n}W^{(m)}_{3, P^{(m)}}}{\hat{\sigma}^{(n,m)}}+\frac{\sqrt{n}W^{(m)}_{4, P^{(m)}}}{\hat{\sigma}^{(n,m)}}+\frac{\sqrt{n} \Omega_{P^{(m)}}^{\textup{RBPT}}}{\hat{\sigma}^{(n,m)}} \geq \tau_\alpha\right] \nonumber\\
    &=\Pr_{P^{(m)}}\left[\frac{\sqrt{n}W^{(m)}_{1, P^{(m)}}}{\sigma_{P^{(m)}}}+\frac{\sqrt{n}W^{(m)}_{2, P^{(m)}}}{\sigma_{P^{(m)}}}+\frac{\sqrt{n}W^{(m)}_{3, P^{(m)}}}{\sigma_{P^{(m)}}}+\frac{\sqrt{n}W^{(m)}_{4, P^{(m)}}}{\sigma_{P^{(m)}}}+\frac{\sqrt{n}\Omega_{P^{(m)}}^{\textup{RBPT}}}{\sigma_{P^{(m)}}} + \tau_\alpha- \tau_\alpha \frac{\hat{\sigma}^{(n,m)}}{\sigma_{P^{(m)}}}\geq \tau_\alpha \right] \nonumber\\
    &=\Pr_{P^{(m)}}\left[\frac{\sqrt{n}W^{(m)}_{1, P^{(m)}}}{\sigma_{P^{(m)}}^{(m)}}\frac{\sigma_{P^{(m)}}^{(m)}}{\sigma_{P^{(m)}}}+\frac{\sqrt{n}W^{(m)}_{2, P^{(m)}}}{\sigma_{P^{(m)}}}+\frac{\sqrt{n}W^{(m)}_{3, P^{(m)}}}{\sigma_{P^{(m)}}}+\frac{\sqrt{n}W^{(m)}_{4, P^{(m)}}}{\sigma_{P^{(m)}}} + \tau_\alpha- \tau_\alpha \frac{\hat{\sigma}^{(n,m)}}{\sigma_{P^{(m)}}^{(m)}}\frac{\sigma_{P^{(m)}}^{(m)}}{\sigma_{P^{(m)}}}\geq \tau_\alpha -\frac{\sqrt{n}\Omega_{P^{(m)}}^{\textup{RBPT}}}{\sigma_{P^{(m)}}}\right] \nonumber\\
    %&=\Pr_{P^{(m)}}\left[\frac{\sqrt{n}W^{(m)}_{1, P^{(m)}}}{\sigma_{P^{(m)}}^{(m)}} \geq \tau_\alpha - \sqrt{\frac{n}{\sigma_{P^{(m)}}^2}}\Omega_{P^{(m)}}^{\textup{RBPT}} \right]+o(1) \label{step:step1_stfr}\\
    &=1-\Phi\left(\tau_\alpha -\sqrt{\frac{n}{\sigma_{P^{(m)}}^2}}\Omega_{P^{(m)}}^{\textup{RBPT}}\right)+o(1)\label{step:step1_rbpt}
\end{align}

Implying that
\begin{align*}
   &\sup_{P\in \cP}\left|\Ex_P[\varphi^{\textup{RBPT}}_\alpha(\cD^{(n)}_{te},\cD_{tr}^{(m)})]-1+\Phi\left(\tau_{\alpha}-\sqrt{\frac{n}{\sigma_P^2}}\Omega_P^{\textup{RBPT}}\right)\right|= o(1) \text{ as }m\to \infty
\end{align*}

\textit{Justifying step \ref{step:step1_rbpt}.} First, from a central limit theorem for triangular arrays \citep[Corollary 9.5.11]{cappe2009inference}, we have that
\[
\sqrt{n}\left(\frac{W^{(m)}_{1, P^{(m)}}}{\sigma_{P^{(m)}}^{(m)}}\right)= \sqrt{n}\left(\frac{\bar{T}^{(n,m)}-\Ex_{P^{(m)}}[T^{(m)}_1 \mid \cD_{tr}^{(m)}]}{\sigma_{P^{(m)}}^{(m)}}\right) = \frac{1}{\sqrt{n}}\sum_{i=1}^n\left(\frac{T_i^{(m)}-\Ex_{P^{(m)}}[T^{(m)}_1 \mid \cD_{tr}^{(m)}]}{\sigma_{P^{(m)}}^{(m)}}\right)\Rightarrow N(0,1)
\]
The conditions for the central limit theorem \citep[Corollary 9.5.11]{cappe2009inference} can be proven to hold like in Theorem \ref{thm:thm1_stfr}'s proof.

Second, we have that
\begin{align*}
   &\frac{\sqrt{n}W^{(m)}_{1, P^{(m)}}}{\sigma_{P^{(m)}}^{(m)}}- \left(\frac{\sqrt{n}W^{(m)}_{1, P^{(m)}}}{\sigma_{P^{(m)}}^{(m)}}\frac{\sigma_{P^{(m)}}^{(m)}}{\sigma_{P^{(m)}}}+\frac{\sqrt{n}W^{(m)}_{2, P^{(m)}}}{\sigma_{P^{(m)}}}+\frac{\sqrt{n}W^{(m)}_{3, P^{(m)}}}{\sigma_{P^{(m)}}}+\frac{\sqrt{n}W^{(m)}_{4, P^{(m)}}}{\sigma_{P^{(m)}}} + \tau_\alpha- \tau_\alpha \frac{\hat{\sigma}^{(n,m)}}{\sigma_{P^{(m)}}^{(m)}}\frac{\sigma_{P^{(m)}}^{(m)}}{\sigma_{P^{(m)}}} \right)=\\
   &=\frac{\sqrt{n}W^{(m)}_{1, P^{(m)}}}{\sigma_{P^{(m)}}^{(m)}}\left(1-\frac{\sigma_{P^{(m)}}^{(m)}}{\sigma_{P^{(m)}}}\right)- \frac{\sqrt{n}W^{(m)}_{2, P^{(m)}}}{\sigma_{P^{(m)}}}-\frac{\sqrt{n}W^{(m)}_{3, P^{(m)}}}{\sigma_{P^{(m)}}}-\frac{\sqrt{n}W^{(m)}_{4, P^{(m)}}}{\sigma_{P^{(m)}}} + \\
   &~~~~ +\tau_\alpha\left(\frac{\hat{\sigma}^{(n,m)}}{\sigma_{P^{(m)}}^{(m)}}-1\right)\left(\frac{\sigma_{P^{(m)}}^{(m)}}{\sigma_{P^{(m)}}}-1\right)+\tau_\alpha\left(\frac{\sigma_{P^{(m)}}^{(m)}}{\sigma_{P^{(m)}}}-1\right)+\tau_\alpha\left(\frac{\hat{\sigma}^{(n,m)}}{\sigma_{P^{(m)}}^{(m)}}-1\right)\\
   &= o_p(1) \text{ as }m\to \infty
\end{align*}

To see why the random quantity above converges to zero in probability, see that because of Assumption \ref{assump:assump3_stfr}, Lemma\footnote{We can apply this STFR's lemma because it still holds when we consider GCM's test statistic.} \ref{lemma:lemma1_stfr}, and continuous mapping theorem, we have that 
\[
\frac{\hat{\sigma}^{(n,m)}}{\sigma_{P^{(m)}}^{(m)}}-1= o_p(1) \text{ and }\frac{\sigma_{P^{(m)}}^{(m)}}{\sigma_{P^{(m)}}}-1= o_p(1) \text{ as }m\to \infty
\]
Additionally, because of Assumptions \ref{assump:assump1_rbpt}, \ref{assump:assump2_rbpt}, and \ref{assump:assump3_rbpt} and condition $n=o(m^{\gamma})$, we have that

\begin{align*}
\left|\frac{\sqrt{n}}{\sigma_{P^{(m)}}}W^{(m)}_{2, P^{(m)}}\right|&=\left|\frac{\sqrt{n}}{\sigma_{P^{(m)}}}\Ex_{P^{(m)}}\left[\ell\left(\int \hat{g}^{(m)}(x,Z_1) d\hat{Q}^{(m)}_{X\mid Z}(x),Y\right)- \ell\left(\int \hat{g}^{(m)}(x,Z_1) dQ^*_{X|Z}(x),Y\right) \mid \cD_{tr}^{(m)}\right]\right|\\
&\leq \frac{\sqrt{n}}{\sigma_{P^{(m)}}}\Ex_{P^{(m)}}\left[  \left|\ell\left(\int \hat{g}^{(m)}(x,Z_1) d\hat{Q}^{(m)}_{X\mid Z}(x),Y\right)- \ell\left(\int \hat{g}^{(m)}(x,Z_1) dQ^*_{X|Z}(x),Y\right)\right| \mid \cD_{tr}^{(m)}\right]\\
&\leq \frac{L\sqrt{n} }{\sigma_{P^{(m)}}} \cdot \Ex_{P^{(m)}}\left[\norm{\int \hat{g}^{(m)}(x,Z_1) d\hat{Q}^{(m)}_{X\mid Z}(x)- \int \hat{g}^{(m)}(x,Z_1) dQ^*_{X|Z}(x)}_2 \mid \cD_{tr}^{(m)}\right]\\
&\leq \frac{L\sqrt{n} }{\sigma_{P^{(m)}}} \cdot \Ex_{P^{(m)}}\left[\norm{\int \hat{g}^{(m)}(x,Z_1) d\hat{Q}^{(m)}_{X\mid Z}(x)- \int \hat{g}^{(m)}(x,Z_1) dQ^*_{X|Z}(x)}_1 \mid \cD_{tr}^{(m)}\right]\\
&\leq \frac{L\sqrt{n} }{\sigma_{P^{(m)}}} \cdot \Ex_{P^{(m)}}\left[\int \norm{\hat{g}^{(m)}(x,Z_1)}_1 \cdot |\hat{q}^{(m)}_{X\mid Z}(x|Z)-q^*_{X|Z}(x|Z)|d\mu(x) \mid \cD_{tr}^{(m)}\right]\\
&\leq \frac{LM\sqrt{n} }{\sigma_{P^{(m)}}} \cdot \Ex_{P^{(m)}}\left[\int |\hat{q}^{(m)}_{X\mid Z}(x|Z)-q^*_{X|Z}(x|Z)| d\mu(x) \mid \cD_{tr}^{(m)}\right]\\
&= \frac{2LM\sqrt{n}}{\inf_{P\in \cP}\sigma_P} \cdot \Ex_{P^{(m)}}\left[ d_{\text{TV}}(\hat{Q}^{(m)}_{X\mid Z},Q^*_{X|Z}) \mid \cD_{tr}^{(m)}\right]\\
&= \frac{2LM}{\inf_{P\in \cP}\sigma_P} \cdot\left(o(m^{\gamma})\cO_{p}(m^{-2\gamma})\right)^{1/2}\\
&= o_{p}(1)
\end{align*}

\begin{align*}
\left|\frac{\sqrt{n}}{\sigma_{P^{(m)}}}W^{(m)}_{3, P^{(m)}}\right|&=\left|\Ex_{P^{(m)}}\left[\ell\left(\int \hat{g}^{(m)}(x,Z_1)  dQ^*_{X|Z}(x),Y\right)- \ell\left(\int g_{P^{(m)}}^*(x,Z_1)  dQ^*_{X|Z}(x),Y\right) \mid \cD_{tr}^{(m)}\right]\right|\\
&\leq \frac{\sqrt{n}}{\sigma_{P^{(m)}}}\Ex_{P^{(m)}}\left[  \left|\ell\left(\int \hat{g}^{(m)}(x,Z_1)  dQ^*_{X|Z}(x),Y\right)- \ell\left(\int g_{P^{(m)}}^*(x,Z_1)  dQ^*_{X|Z}(x),Y\right) \right| \mid \cD_{tr}^{(m)}\right]\\
&\leq \frac{L\sqrt{n}}{\sigma_{P^{(m)}}} \cdot \Ex_{P^{(m)}}\left[\norm{\int \hat{g}^{(m)}(x,Z_1)  dQ^*_{X|Z}(x)- \int g^*_{P^{(m)}}(x,Z_1)  dQ^*_{X|Z}(x)}_2 \mid \cD_{tr}^{(m)}\right]\\
&= \frac{L\sqrt{n}}{\sigma_{P^{(m)}}} \cdot \Ex_{P^{(m)}}\left[\norm{\int \hat{g}^{(m)}(x,Z_1) - g^*_{P^{(m)}}(x,Z_1)  dQ^*_{X|Z}(x)}_2 \mid \cD_{tr}^{(m)}\right]\\
&\leq \frac{L\sqrt{n}}{\sigma_{P^{(m)}}} \cdot \Ex_{P^{(m)}}\left[\int \norm{\hat{g}^{(m)}(x,Z_1) - g^*_{P^{(m)}}(x,Z_1)}_2  dQ^*_{X|Z}(x) \mid \cD_{tr}^{(m)}\right]\\
&= \frac{L\sqrt{n}}{\sigma_{P^{(m)}}} \cdot \Ex_{P^{(m)}}\left[\int \norm{\hat{g}^{(m)}(x,Z_1) - g^*_{P^{(m)}}(x,Z_1)}_2  \frac{dQ^*_{X|Z}}{dP_{X\mid Z}}(x) dP_{X\mid Z}(x) \mid \cD_{tr}^{(m)}\right]\\
&= \frac{L\sqrt{n}}{\sigma_{P^{(m)}}} \cdot \Ex_{P^{(m)}}\left[\norm{\hat{g}^{(m)}(X_1,Z_1) - g^*_{P^{(m)}}(X_1,Z_1)}_2  \frac{dQ^*_{X|Z}}{dP_{X\mid Z}}(X_1)  \mid \cD_{tr}^{(m)}\right]\\
&\leq \frac{L\sqrt{n}}{\sigma_{P^{(m)}}} \cdot \left(\Ex_{P^{(m)}}\left[\norm{\hat{g}^{(m)}(X_1,Z_1) - g^*_{P^{(m)}}(X_1,Z_1)}^2_2  \mid \cD_{tr}^{(m)}\right] \Ex_{P^{(m)}}\left[\left(\frac{dQ^*_{X|Z}}{dP_{X\mid Z}}(X_1)\right)^2 \right]\right)^{1/2}\\
&= \frac{L\sqrt{n}}{\sigma_{P^{(m)}}} \cdot \left(\Ex_{P^{(m)}}\left[\norm{\hat{g}^{(m)}(X_1,Z_1) - g^*_{P^{(m)}}(X_1,Z_1)}^2_2  \mid \cD_{tr}^{(m)}\right] \Ex_{P^{(m)}}\left[\int\frac{dQ^*_{X|Z}}{dP_{X\mid Z}}(x) dQ^*_{X|Z}(x) \right]\right)^{1/2}\\
&= \frac{L\sqrt{n}}{\sigma_{P^{(m)}}} \cdot \left(\Ex_{P^{(m)}}\left[\norm{\hat{g}^{(m)}(X_1,Z_1) - g^*_{P^{(m)}}(X_1,Z_1)}^2_2  \mid \cD_{tr}^{(m)}\right] \Ex_{P^{(m)}}\left[\chi^2\left(Q^*_{X|Z}||P_{X\mid Z}\right) +1\right]\right)^{1/2}\\
&\leq \frac{LR\sqrt{n}}{\inf_{P\in \cP}\sigma_P} \cdot\left(\Ex_{P^{(m)}}\left[\norm{\hat{g}^{(m)}(X_1,Z_1) - g^*_{P^{(m)}}(X_1,Z_1)}^2_2  \mid \cD_{tr}^{(m)}\right]\right)^{1/2}\\
&= \frac{LR}{\inf_{P\in \cP}\sigma_P} \cdot\left(o(m^{\gamma})\cO_{p}(m^{-\gamma})\right)^{1/2}\\
&= o_{p}(1)
\end{align*}

\begin{align*}
\left|\frac{\sqrt{n}}{\sigma_{P^{(m)}}}W^{(m)}_{4, P^{(m)}}\right|&=\left|\Ex_{P^{(m)}}\left[\ell\left(\hat{g}^{(m)}(X_1,Z_1),Y_1\right)- \ell\left( g_{P^{(m)}}^*(X_1,Z_1),Y_1\right) \mid \cD_{tr}^{(m)}\right]\right|\\
&\leq \frac{\sqrt{n}}{\sigma_{P^{(m)}}}\Ex_{P^{(m)}}\left[\left|\ell\left(\hat{g}^{(m)}(X_1,Z_1),Y_1\right)- \ell\left( g_{P^{(m)}}^*(X_1,Z_1),Y_1\right)\right| \mid \cD_{tr}^{(m)}\right]\\
&\leq \frac{L\sqrt{n}}{\sigma_{P^{(m)}}} \cdot \Ex_{P^{(m)}}\left[\norm{\hat{g}^{(m)}(X_1,Z_1)-g_{P^{(m)}}^*(X_1,Z_1)}_2 \mid \cD_{tr}^{(m)}\right]\\
&\leq  \frac{L\sqrt{n}}{\inf_{P\in \cP}\sigma_P} \cdot \left(\Ex_{P^{(m)}}\left[ \norm{\hat{g}^{(m)}(X_1,Z_1) - g^*_{P^{(m)}}(X_1,Z_1)}^2_2 \mid \cD_{tr}^{(m)}\right]\right)^{1/2}\\
&= \frac{L}{\inf_{P\in \cP}\sigma_P} \cdot\left(o(m^{\gamma})\cO_{p}(m^{-\gamma})\right)^{1/2}\\
&= o_{p}(1)
\end{align*}

where $M$ is an upper bound for the sequence $\left(\norm{\hat{g}^{(m)}(x,z)}_1\right)_{m\in\mathbb{N}}$ (Assumption \ref{assump:assump3_rbpt}) and $R$ is an upper bound for the sequence $\left((\Ex_{P^{(m)}}\left[\chi^2\left(Q^*_{X|Z}||P_{X\mid Z}\right) +1\right])^{1/2}\right)_{m\in\mathbb{N}}$  (Assumption \ref{assump:assump2_rbpt}).

Finally, 
\begin{align*}
    &\frac{\sqrt{n}W^{(m)}_{1, P^{(m)}}}{\sigma_{P^{(m)}}^{(m)}}\frac{\sigma_{P^{(m)}}^{(m)}}{\sigma_{P^{(m)}}}+\frac{\sqrt{n}W^{(m)}_{2, P^{(m)}}}{\sigma_{P^{(m)}}}+\frac{\sqrt{n}W^{(m)}_{3, P^{(m)}}}{\sigma_{P^{(m)}}}+\frac{\sqrt{n}W^{(m)}_{4, P^{(m)}}}{\sigma_{P^{(m)}}} + \tau_\alpha- \tau_\alpha \frac{\hat{\sigma}^{(n,m)}}{\sigma_{P^{(m)}}^{(m)}}\frac{\sigma_{P^{(m)}}^{(m)}}{\sigma_{P^{(m)}}}=\\
    &=\frac{\sqrt{n}W^{(m)}_{1, P^{(m)}}}{\sigma_{P^{(m)}}^{(m)}} - \left[ \frac{\sqrt{n}W^{(m)}_{1, P^{(m)}}}{\sigma_{P^{(m)}}^{(m)}}- \left(\frac{\sqrt{n}W^{(m)}_{1, P^{(m)}}}{\sigma_{P^{(m)}}^{(m)}}\frac{\sigma_{P^{(m)}}^{(m)}}{\sigma_{P^{(m)}}}+\frac{\sqrt{n}W^{(m)}_{2, P^{(m)}}}{\sigma_{P^{(m)}}}+\frac{\sqrt{n}W^{(m)}_{3, P^{(m)}}}{\sigma_{P^{(m)}}}+\frac{\sqrt{n}W^{(m)}_{4, P^{(m)}}}{\sigma_{P^{(m)}}} + \tau_\alpha- \tau_\alpha \frac{\hat{\sigma}^{(n,m)}}{\sigma_{P^{(m)}}^{(m)}}\frac{\sigma_{P^{(m)}}^{(m)}}{\sigma_{P^{(m)}}} \right) \right]\\
    &=\frac{\sqrt{n}W^{(m)}_{1, P^{(m)}}}{\sigma_{P^{(m)}}^{(m)}} + o_p(1)\Rightarrow N(0,1)
\end{align*}

by Slutsky's theorem. Because $N(0,1)$ is a continuous distribution, we have uniform convergence of the distribution function \citep{resnick2019probability}[Chapter 8, Exercise 5], and we do not have to worry about the fact that $\tau_\alpha -\frac{\sqrt{n}\Omega_{P^{(m)}}^{\textup{RBPT}}}{\sigma_{P^{(m)}}}$ depends on $m$.

\end{proof}

\newpage
\section{Experiments}\label{append:exp}

We include extra experiments in which $d_Z\in\{10,20,30,40\}$ and $Y\mid X,Z$ has skewed normal distributions with location $\mu=cX+a^\top Z + \gamma (b^\top Z)^2$, scale $\sigma=1$, and shape $s\in\{0,3\}$ (shape $s=0$ lead to the normal distribution). We can see that when $d_Z=40$, RBPT2 fails to control Type-I error. This specific case can be corrected by increasing the training set size.

\begin{figure}[h]
    \centering
    \hspace{-.55cm}
    \renewcommand{\arraystretch}{0}
    \begin{tabular}{c}
        \includegraphics[width=.6\textwidth]{Neurips_2023/figs/exp1_10_0_mse.png}\\[.0em]
        \includegraphics[width=.6\textwidth]{Neurips_2023/figs/exp1_20_0_mse.png}\\[.0em]
        \includegraphics[width=.6\textwidth]{Neurips_2023/figs/exp1_30_0_mse.png}\\[.0em]
        \includegraphics[width=.6\textwidth]{Neurips_2023/figs/exp1_40_0_mse.png}\\[.0em]
    \end{tabular}
    \caption{\small Skewness $s=0$.}
    \label{fig:}
    \vspace{-.25cm}
\end{figure}


\begin{figure}[h]
    \centering
    \hspace{-.55cm}
    \renewcommand{\arraystretch}{0}
    \begin{tabular}{c}
        \includegraphics[width=.6\textwidth]{Neurips_2023/figs/exp1_10_3_mse.png}\\[.0em]
        \includegraphics[width=.6\textwidth]{Neurips_2023/figs/exp1_20_3_mse.png}\\[.0em]
        \includegraphics[width=.6\textwidth]{Neurips_2023/figs/exp1_30_3_mse.png}\\[.0em]
        \includegraphics[width=.6\textwidth]{Neurips_2023/figs/exp1_40_3_mse.png}\\[.0em]
    \end{tabular}
    \caption{\small Skewness $s=3$.}
    \label{fig:}
    \vspace{-.25cm}
\end{figure}

==> sections/todo.tex <==
\section{TO-DOs}
\begin{itemize}
    %\item Double robustness comments.
    %\item How do you see our theoretical results?
    %\item Include definition of test o level $\alpha$
    \item Include new experiments and other suggestions made by reviewers.
    %\item Include references for assumptions on convergence rates.
    \item Maybe assumption \ref{assump:assump3_stfr} comes for free when we make assump \ref{assump:assump1_stfr} (Felipe).
    %\item Remarks about universal approximations (Yuekai). 
    \item Write conclusion (Felipe).
    %\item domain lipz resit
    %\item make it clear that $\epsilon$ and $\eta$ depend on $P$ and check if any proof need to be changed
    %\item support of integrand can be very large (use diameter of B and assumpt to bound the size of f's and g's)
\end{itemize}
